Quantum Multiplexers, Parrondo Games, and Proper Quantization

A quantum logic gate of particular interest to both electrical engineers and game theorists is the quantum multiplexer. This shared interest is due to the facts that an arbitrary quantum logic gate may be expressed, up to arbitrary accuracy, via a circuit consisting entirely of variations of the quantum multiplexer, and that certain one player games, the history dependent Parrondo games, can be quantized as games via a particular variation of the quantum multiplexer. However, to date all such quantizations have lacked a certain fundamental game theoretic property. The main result in this dissertation is the development of quantizations of history dependent quantum Parrondo games that satisfy this fundamental game theoretic property. Our approach also yields fresh insight as to what should be considered as the proper quantum analogue of a classical Markov process and gives the first game theoretic measures of multiplexer behavior.

==> Chapter4.tex <==
% Converted from Microsoft Word to LaTeX
% by Chikrii Softlab Word2TeX converter (version 3.0)
% Copyright (C) 1999-2003 Chikrii Softlab. All rights reserved.
% http://www.chikrii.com
% mailto: info@chikrii.com
% License: CSL#0036C0
%
%\documentclass[12pt]{article}
%\usepackage{latexsym}
%\usepackage{amssymb}
%\usepackage{amsmath}
%\usepackage{color}
%\usepackage{graphicx}
% \usepackage{setspace}
% \usepackage{amsthm}
%\doublespacing
%
%\begin{document}
\chapter{Quaternionic Coordinatization of 2 Player, 2 Strategy Quantum Games}

This chapter presents an expository review of the work of Landsburg \cite{Landsburg} on the quaternionic coordinatization of two player, two strategy games quantized via the EWL protocol \cite{Eisert} with the initial state 
$$
\frac{1}{\sqrt{2}}\left(\left|00\right\rangle+\left|11\right\rangle\right).
$$
Landsburg's work leads to a quaternionic computational framework that allows for the identification and classification of the potential Nash equilibria. The exposition offered here is relevant to the discussion in chapter 5 of the joint work by A. Ahmed, S. Bleiler, and F. S. Khan on an octonionic coordinatization of three player, two strategy quantum games quantized a la EWL protocol and played with initial state 
$$
\frac{1}{\sqrt{2}}\left(\left|000\right\rangle+\left|111\right\rangle\right)
$$
with the goal of providing an octonionic computational framework that will allow for the identification and classification of the potential Nash equilibria. Quaternions are discussed in some detail in appendix 1.

In \cite{Landsburg}, the two classical pure 
strategies available to the players are represented in the quantized game by the $SU(2)$ matrices {\it no flip} ($N$) and {\it flip} ($F$) respectively indicated in (1),
\begin{equation}
\label{eq1}
\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill \\
 0 \hfill & 1 \hfill \\
\end{array} }} \right),\mbox{ }\left( {{\begin{array}{*{20}c}
 0 \hfill & \eta \hfill \\
 {-\bar {\eta }} \hfill & 0 \hfill \\
\end{array} }} \right)
\end{equation}
where the unit complex number $\eta $ is chosen such that the four outcome states of 
our two player game forms an orthogonal basis of the state 
space $\mathbb{C}P^4$, with standard basis $\left\{ {\left| {00} \right\rangle 
,\left| {01} \right\rangle ,\left| {10} \right\rangle ,\left| {11} 
\right\rangle } \right\}$. These four outcome states are denoted by \textit{NN}, \textit{NF}, 
\textit{FN}, \textit{FF}, where any of these pairs of $N $ and $F$ represent the pure strategy choices of 
the players I and II, respectively. A direct calculation shows for orthogonality of the 
outcome states, by necessity $\eta ^8=1$, so setting 
$$
\eta =\frac{1+i}{\sqrt 2 }
$$
makes the four states \textit{NN}, \textit{NF}, \textit{FN}, \textit{FF} mutually orthogonal. As described above, a pure 
quantum strategy for each player corresponds to a general element of 
$SU(2)$ acting on a player's qubit before the player sends it to the referee, and as described above a classical pure strategy corresponds to the player's choice of one of the 
matrices $N$ or $F$ given above for these actions on their qubits.
%
%Either taking a mixture, a superposition, or a mixed superposition of the 
%pure strategies produces a probability distribution over the four outcomes 
%of the game. The expected value for each pair of strategic choices by the 
%players forms the set of payoffs for the game. 
Exploiting the identification of $SU(2)$ with the unit quaternions, and after identifying each pure 
quantum strategy for each player with a suitable unit quaternion $p$ or $q$, Landsburg shows that 
the probability distribution over the four possible outcomes when the 
players use these strategies is then given by the squares of the 
coefficients of the unit quaternion \textit{pq}. 

This corresponds in the Bleiler formalism to a map $L$ from $\prod Q_i$ to $\Delta(ImG)$ as shown in the Figure \ref{L map} below. When mixed quantum strategies are played, the map $L$ induces a coordinatization of the map $G^{{\cal{Q}}_{I}}_{*}$ from $\Delta(\prod Q_i)$ to $\Delta(ImG^{{\cal{Q}}_{I}})$. We denote this coordinatized map by $L_{*}$. These maps give Landsburg the computational capability to recognize and classify the potential Nash equilibria of $G^{{\cal{Q}}_{I}}$ and $G^{m{\cal{Q}}_{I}}$. In particular, for zero-sum games $G$ he shows that in the game $G^{m{\cal{Q}}_{I}}$ the players can guarantee to themselves the average of the four possible outcomes of the game $G$ \cite{Landsburg}. Frequently, this is a superior equilibrium payoff than that available to the players restricted to using classical mixed strategies. 

\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.45]{fig1.jpg}
\caption{Landsburg's maps $L$ and $L_{*}$.}
\label{L map}
\end{center}
\end{figure}

\section{Quaternionization}

A pure quantum strategy for each player can be represented by a matrix 
in $SU(2)\cong S^3\cong SP(1)$, the group of unit quaternions. Each player communicates his strategic choice to a referee via a 
qubit in superposition. The referee initially sends to the two players qubits 
in the maximally entangled state 
$$
M=\frac{1}{\sqrt 2}\left[\left| {00} \right\rangle +\left| {11} 
\right\rangle\right].
$$
The two classical pure strategies available to the players 
are \textit{flip} denoted by $F$, and \textit{no flip} denoted by $N$, represented respectively by 
the $SU(2)$matrices
\[
F=\left( {{\begin{array}{*{20}c}
 0 \hfill & \eta \hfill \\
 {-\bar {\eta }} \hfill & 0 \hfill \\
\end{array} }} \right),\mbox{ } 
N=\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill \\
 0 \hfill & 1 \hfill \\
\end{array} }} \right)
\]
where $\eta \in U(1)$ is chosen such that the four outcome states 
$$
\mathcal{B}_{FN}=\left\{NN, NF, FN, FF \right\}
$$
of our two player game form an orthogonal basis of the state space $\mathbb{C}^4$, which carries the  
computational basis 
$$
\mathcal{B}=\left\{ {\left| {00} \right\rangle ,\left| {01} \right\rangle 
,\left| {10} \right\rangle ,\left| {11} \right\rangle } \right\}.
$$
Call $\mathcal{B}_{FN}$ the {\it outcome basis}. Any of the pairs of $N$ and $F$ in $\mathcal{B}_{FN}$ represent the pure strategy choices of the players 1 and 2 respectively. 
A direct calculation shows that $\eta ^8=1$, so setting
$$
\eta 
=\frac{1+i}{\sqrt 2 }
$$ 
makes the four elements of $\mathcal{B}_{FN}$ orthogonal. A pure quantum strategy for each player now 
corresponds to a general element of $SU(2)$ that acts on a player's qubit before 
the player sends it to the referee. A classical pure strategy corresponds to 
the player's choice of one of the matrices $F$ or $N$ given above for these 
actions on their qubits.

Either taking a mixture, a superposition, or a mixed superposition of the 
pure strategies produces a probability distribution over the four outcomes 
of the game. The expected value for each pair of strategic choices by the 
players forms the set of payoffs for the game. After identifying each pure 
quantum strategy, i.e each superposition of the classical pure strategies, 
for each player with a suitable unit quaternion $p$ or $q$, Landsburg shows that 
the probability distribution over the four possible outcomes when the 
players use these strategies is then given by the squares of the 
coefficients of the unit quaternion \textit{pq}. Note that the superpositions include 
the mixtures. From this, Landsburg is able to obtain payoff expressions for 
when the players use mixtures, superpositions, or mixed superpositions of 
the pure classical strategies. Using these expressions, Landsburg can 
classify the Nash equilibria of the maximally entangled quantum game, and 
for zero sum games, can show that by using mixed superpositions of 
strategies, the players can guarantee to themselves the average of the four 
possible outcomes. Frequently, this is a superior equilibrium than that 
available to players restricted to classical mixed strategies.

\subsection{The Game State}

Suppose each player is given access to a qubit each and the two qubits are maximally 
entangled. Again, this is the state
$$
M=\frac{1}{\sqrt{2}}\left| 00 
\right\rangle +\left| 11 \right\rangle 
$$
which in the standard basis of $\mathbb{C}^2$ is expressed as 
$$
\frac{1}{\sqrt{2}}\left( {{\begin{array}{*{20}c}
 1 \hfill \\
 0 \hfill \\
 0 \hfill \\
 1 \hfill \\
\end{array} }} \right)
$$

Let the strategies of the two players be 
$$
S=\left( {{\begin{array}{*{20}c}
 A \hfill & B \hfill \\
 {-\bar {B}} \hfill & {\bar {A}} \hfill \\
\end{array} }} \right), \quad T=\left( {{\begin{array}{*{20}c}
 P \hfill & Q \hfill \\
 {-\bar {Q}} \hfill & {\bar {P}} \hfill \\
\end{array} }} \right)
$$ 
respectively. Then the ``joint'' strategy matrix 
acting on the joint state vector of the two initial qubits is 
\[
S \otimes T =\left( {{\begin{array}{*{20}c}
 A \hfill & B \hfill \\
 {-\bar {B}} \hfill & {\bar {A}} \hfill \\
\end{array} }} \right)\otimes \left( {{\begin{array}{*{20}c}
 P \hfill & Q \hfill \\
 {-\bar {Q}} \hfill & {\bar {P}} \hfill \\
\end{array} }} \right)=\left( {{\begin{array}{*{20}c}
 {AP} \hfill & {AQ} \hfill & {BP} \hfill & {BQ} \hfill \\
 {-A\bar {Q}} \hfill & {A\bar {P}} \hfill & {-B\bar {Q}} \hfill & {B\bar 
{P}} \hfill \\
 {-\bar {B}P} \hfill & {-\bar {B}Q} \hfill & {\bar {A}P} \hfill & {\bar 
{A}Q} \hfill \\
 {\bar {B}\bar {Q}} \hfill & {-\bar {B}\bar {P}} \hfill & {-\bar {A}\bar 
{Q}} \hfill & {\bar {A}\bar {P}} \hfill \\
\end{array} }} \right)% {\begin{array}{*{20}c}
% {HH} \hfill \\
% {HT} \hfill \\
% {TH} \hfill \\
% {TT} \hfill \\
%\end{array} }
\]
The action of this matrix on the initial state vector $M$ is 
\begin{equation}\label{game state}
\frac{1}{\sqrt{2}}\left( {{\begin{array}{*{20}c}
 {AP} \hfill & {AQ} \hfill & {BP} \hfill & {BQ} \hfill \\
 {-A\bar {Q}} \hfill & {A\bar {P}} \hfill & {-B\bar {Q}} \hfill & {B\bar 
{P}} \hfill \\
 {-\bar {B}P} \hfill & {-\bar {B}Q} \hfill & {\bar {A}P} \hfill & {\bar 
{A}Q} \hfill \\
 {\bar {B}\bar {Q}} \hfill & {-\bar {B}\bar {P}} \hfill & {-\bar {A}\bar 
{Q}} \hfill & {\bar {A}\bar {P}} \hfill \\
\end{array} }} \right)\left( {{\begin{array}{*{20}c}
 1 \hfill \\
 0 \hfill \\
 0 \hfill \\
 1 \hfill \\
\end{array} }} \right)%{\begin{array}{*{20}c}
% {HH} \hfill \\
% {HT} \hfill \\
% {TH} \hfill \\
% {TT} \hfill \\
%\end{array} }
=\frac{1}{\sqrt{2}}\left( {{\begin{array}{*{20}c}
 {AP+BQ} \hfill \\
 {-A\bar {Q}+B\bar {P}} \hfill \\
 {-\bar {B}P+\bar {A}Q} \hfill \\
 {\bar {B}\bar {Q}+\bar {A}\bar {P}} \hfill \\
\end{array} }} \right)%{\begin{array}{*{20}c}
% {HH} \hfill \\
% {HT} \hfill \\
% {TH} \hfill \\
% {TT} \hfill \\
%\end{array} }
\end{equation}
Call the right hand side of equation (\ref{game state}) the {\it game state}.

\subsection{From Computational to the Outcome Basis}

Note that the game state in equation (\ref{game state}) is expressed in the computational basis. However, if we make a measurement of the game state with respect to the computational basis, the resulting probability distribution will be over the various configurations of $H$ and $T$. This distribution is useless for computing the expected payoff to the players, which in fact requires a probability distribution over the various configurations of the strategic choices of the two players, namely, $N$ and $F$. Therefore, a basis change from the computational $\left\{H,T\right\}$ basis to outcome $\left\{N,F\right\}$ basis is required.

The change of basis matrix from the $\left\{H,T\right\}$ basis to $\left\{N,F\right\}$ basis is
computed as follows. First, represent the $\left\{N,F\right\}$ basis in terms of the $\left\{H,T\right\}$
basis by computing the action of the matrices representing $F$ and $N$ on the initial state $M$
in the $\left\{H,T\right\}$ basis. The ``joint'' matrices are:
$$
 N\otimes N=NN=\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill \\
 0 \hfill & 1 \hfill \\
\end{array} }} \right)\otimes \left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill \\
 0 \hfill & 1 \hfill \\
\end{array} }} \right)=\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 1 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 1 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & 1 \hfill \\
\end{array} }} \right)
$$
$$
 F\otimes N=FN=\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill \\
 0 \hfill & 1 \hfill \\
\end{array} }} \right)\otimes \left( {{\begin{array}{*{20}c}
 0 \hfill & \eta \hfill \\
 {-\bar {\eta }} \hfill & 0 \hfill \\
\end{array} }} \right)=\left( {{\begin{array}{*{20}c}
 0 \hfill & \eta \hfill & 0 \hfill & 0 \hfill \\
 {-\bar {\eta }} \hfill & 0 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & \eta \hfill \\
 0 \hfill & 0 \hfill & {-\bar {\eta }} \hfill & 0 \hfill \\
\end{array} }} \right) 
$$
$$
 N\otimes F=NF=\left( {{\begin{array}{*{20}c}
 0 \hfill & \eta \hfill \\
 {-\bar {\eta }} \hfill & 0 \hfill \\
\end{array} }} \right)\otimes \left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill \\
 0 \hfill & 1 \hfill \\
\end{array} }} \right)=\left( {{\begin{array}{*{20}c}
 0 \hfill & 0 \hfill & \eta \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & \eta \hfill \\
 {-\bar {\eta }} \hfill & 0 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & {-\bar {\eta }} \hfill & 0 \hfill & 0 \hfill \\
\end{array} }} \right) 
$$
$$
 F\otimes F=FF=\left( {{\begin{array}{*{20}c}
 0 \hfill & \eta \hfill \\
 {-\bar {\eta }} \hfill & 0 \hfill \\
\end{array} }} \right)\otimes \left( {{\begin{array}{*{20}c}
 0 \hfill & \eta \hfill \\
 {-\bar {\eta }} \hfill & 0 \hfill \\
\end{array} }} \right)=\left( {{\begin{array}{*{20}c}
 0 \hfill & 0 \hfill & 0 \hfill & {\eta ^2} \hfill \\
 0 \hfill & 0 \hfill & {-\eta \bar {\eta }} \hfill & 0 \hfill \\
 0 \hfill & {-\bar {\eta }\eta } \hfill & 0 \hfill & 0 \hfill \\
 {\bar {\eta }^2} \hfill & 0 \hfill & 0 \hfill & 0 \hfill \\
\end{array} }} \right) \\ 
$$
and their action on the initial state $M$ in the $\left\{H,T\right\}$ basis gives:
\[
%\begin{array}{l}
NN(M): \frac{1}{\sqrt{2}}\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 1 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 1 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & 1 \hfill \\
\end{array} }} \right)\left( {{\begin{array}{*{20}c}
 1 \hfill \\
 0 \hfill \\
 0 \hfill \\
 1 \hfill \\
\end{array} }} \right)
=\frac{1}{\sqrt{2}}\left( {{\begin{array}{*{20}c}
 1 \hfill \\
 0 \hfill \\
 0 \hfill \\
 1 \hfill \\
\end{array} }} \right)
\]
%=\frac{1}{\sqrt{2}}\left[\left| {HH} \right\rangle +\left| {TT} \right\rangle\right] \\ 
\[
FN(M): \frac{1}{\sqrt{2}}\left( {{\begin{array}{*{20}c}
 0 \hfill & \eta \hfill & 0 \hfill & 0 \hfill \\
 {-\bar {\eta }} \hfill & 0 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & \eta \hfill \\
 0 \hfill & 0 \hfill & {-\bar {\eta }} \hfill & 0 \hfill \\
\end{array} }} \right)\left( {{\begin{array}{*{20}c}
 1 \hfill \\
 0 \hfill \\
 0 \hfill \\
 1 \hfill \\
\end{array} }} \right)
=\frac{1}{\sqrt{2}}\left( {{\begin{array}{*{20}c}
 0 \hfill \\
 {-\bar {\eta }} \hfill \\
 \eta \hfill \\
 0 \hfill \\
\end{array} }} \right)
%=\frac{1}{\sqrt{2}}\left[-\bar {\eta }\left| {HT} \right\rangle +\eta \left| {TH} 
%\right\rangle \right] \\ 
% \end{array}
\]
\[
%\begin{array}{l}
 \\ 
NF(M): =\frac{1}{\sqrt{2}}\left( {{\begin{array}{*{20}c}
 0 \hfill & 0 \hfill & \eta \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & \eta \hfill \\
 {-\bar {\eta }} \hfill & 0 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & {-\bar {\eta }} \hfill & 0 \hfill & 0 \hfill \\
\end{array} }} \right)\left( {{\begin{array}{*{20}c}
 1 \hfill \\
 0 \hfill \\
 0 \hfill \\
 1 \hfill \\
\end{array} }} \right)
=\frac{1}{\sqrt{2}}\left( {{\begin{array}{*{20}c}
 0 \hfill \\
 \eta \hfill \\
 {-\bar {\eta }} \hfill \\
 0 \hfill \\
\end{array} }} \right)
\]
%=\frac{1}{\sqrt{2}}\left[\eta \left| {HT} \right\rangle -\bar {\eta }\left| {TH} 
%\right\rangle\right] \\ 
\[
FF(M): =\frac{1}{\sqrt{2}}\left( {{\begin{array}{*{20}c}
 0 \hfill & 0 \hfill & 0 \hfill & {\eta ^2} \hfill \\
 0 \hfill & 0 \hfill & {-\eta \bar {\eta }} \hfill & 0 \hfill \\
 0 \hfill & {-\bar {\eta }\eta } \hfill & 0 \hfill & 0 \hfill \\
 {\bar {\eta }^2} \hfill & 0 \hfill & 0 \hfill & 0 \hfill \\
\end{array} }} \right)\left( {{\begin{array}{*{20}c}
 1 \hfill \\
 0 \hfill \\
 0 \hfill \\
 1 \hfill \\
\end{array} }} \right)
=\frac{1}{\sqrt{2}}\left( {{\begin{array}{*{20}c}
 {\eta ^2} \hfill \\
 0 \hfill \\
 0 \hfill \\
 {\bar {\eta }^2} \hfill \\
\end{array} }} \right)
%=\frac{1}{\sqrt{2}}\left[\eta ^2\left| {HH} \right\rangle +\bar {\eta }^2\left| {TT} 
%\right\rangle =i\left| {HH} \right\rangle -i\left| {TT} \right\rangle \right] \\ 
% \end{array}
\]
In short:
\[
 NN=\frac{1}{\sqrt{2}}\left[\left| {HH} \right\rangle +\left| {TT} \right\rangle\right]
 \]
 \[
 FN=\frac{1}{\sqrt{2}}\left[-\bar {\eta }\left| {HT} \right\rangle +\eta \left| {TH} \right\rangle\right] 
\]
\[ 
 NF=\frac{1}{\sqrt{2}}\left[\eta \left| {HT} \right\rangle -\bar {\eta }\left| {TH} \right\rangle\right] 
 \]
 \[
 FF=\frac{1}{\sqrt{2}}\left[i\left| {HH} \right\rangle -i\left| {TT} \right\rangle\right] \\ 
\]
Therefore, the basis change matrix from the F/N basis to H/T basis is 
\[
\begin{array}{l}
 %{\begin{array}{*{20}c}
% {NN} \hfill & {FN} \hfill & {NF} \hfill & {FF} \hfill \\
%\end{array} } \\ 
 X=\frac{1}{\sqrt 2 }\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill & 0 \hfill & i \hfill \\
 0 \hfill & {-\bar {\eta }} \hfill & \eta \hfill & 0 \hfill \\
 0 \hfill & \eta \hfill & {-\bar {\eta }} \hfill & 0 \hfill \\
 1 \hfill & 0 \hfill & 0 \hfill & {-i} \hfill \\
\end{array} }} \right)%{\begin{array}{*{20}c}
% {HH} \hfill \\
% {HT} \hfill \\
% {TH} \hfill \\
% {TT} \hfill \\
%\end{array} } \\ 
 \end{array}.
\]
Because $X$ is unitary, it follows that the change of basis matrix from H/T to F/N basis is just
\[
X^{-1}=\frac{1}{\sqrt 2 }\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill & 0 \hfill & 1 \hfill \\
 0 \hfill & {-\eta } \hfill & {\bar {\eta }} \hfill & 0 \hfill \\
 0 \hfill & {\bar {\eta }} \hfill & {-\eta } \hfill & 0 \hfill \\
 {-i} \hfill & 0 \hfill & 0 \hfill & i \hfill \\
\end{array} }} \right)
\]
We can now express the game state in the F/N basis as follows. 
\begin{align*}
\frac{1}{\sqrt 2 }\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill & 0 \hfill & 1 \hfill \\
 0 \hfill & {-\eta } \hfill & {\bar {\eta }} \hfill & 0 \hfill \\
 0 \hfill & {\bar {\eta }} \hfill & {-\eta } \hfill & 0 \hfill \\
 {-i} \hfill & 0 \hfill & 0 \hfill & i \hfill \\
\end{array} }} \right)&\frac{1}{\sqrt 2 }\left( {{\begin{array}{*{20}c}
 {AP+BQ} \hfill \\
 {-A\bar {Q}+B\bar {P}} \hfill \\
 {-\bar {B}P+\bar {A}Q} \hfill \\
 {\bar {B}\bar {Q}+\bar {A}\bar {P}} \hfill \\
\end{array} }} \right) \\
&=\frac{1}{2}\left( {{\begin{array}{*{20}c}
 {(AP+BQ)+(\bar {B}\bar {Q}+\bar {A}\bar {P})} \hfill \\
 {-\eta (-A\bar {Q}+B\bar {P})+\bar {\eta }(-\bar {B}P+\bar {A}Q)} \hfill \\
 {\bar {\eta }(-A\bar {Q}+B\bar {P})-\eta (-\bar {B}P+\bar {A}Q)} \hfill \\
 {-i(AP+BQ)+i(\bar {B}\bar {Q}+\bar {A}\bar {P})} \hfill \\
\end{array} }} \right)
\end{align*}

\subsection{Complex Coordinatization of the Payoff Function}

As per the axioms of quantum mechanics, up to phase, the referee observing the game state in the 
outcome basis sees the each basis state according to the following probability distribution.
\[
\begin{array}{l}
 {\rm Prob}(NN)= \frac{1}{4}\left[(AP+BQ)+(\bar {B}\bar {Q}+\bar {A}\bar {P})\right]^2 \\ 
 \\ 
{\rm Prob}(NF)= \frac{1}{4}\left[-\eta (-A\bar {Q}+B\bar {P})+\bar {\eta }(-\bar {B}P+\bar {A}Q)\right]^2 \\ 
 \\ 
{\rm Prob}(FN)=\frac{1}{4}\left[\bar {\eta }(-A\bar {Q}+B\bar {P})-\eta (-\bar {B}P+\bar {A}Q)\right]^2 \\ 
 \\ 
{\rm Prob}(FF)=\frac{1}{4}\left[-i(AP+BQ)+i(\bar {B}\bar {Q}+\bar {A}\bar {P})\right]^2 \\ 
 \end{array}
\]
This distribution defines the payoff function of the game, on which we now put complex co-ordinates as follows. 
%\[
%\begin{array}{l}
% \frac{1}{\sqrt 2 }\left[ {(AP+BQ)+(\bar {B}\bar {Q}+\bar {A}\bar {P})} 
%\right]NN+\frac{1}{\sqrt 2 }\left[ {-\eta (-A\bar {Q}+B\bar {P})+\bar {\eta 
%}(-\bar {B}P+\bar {A}Q)} \right]NF \\ 
% +\frac{1}{\sqrt 2 }\left[ {\bar {\eta }(-A\bar {Q}+B\bar {P})-\eta (-\bar 
%{B}P+\bar {A}Q)} \right]FN+\frac{1}{\sqrt 2 }\left[ {-i(AP+BQ)+i(\bar 
%{B}\bar {Q}+\bar {A}\bar {P})} \right]FF \\ 
% \end{array}
%\]

Let 
$$
A=(A_0 +A_1 i), \quad B=(B_0 +B_1 i)
$$
$$
P=(P_0 +P_1 i), \quad Q=(Q_0 +Q_1 i).
$$ 
Then 
\begin{align*}
&(AP+BQ)\\
&=(A_0 +A_1 i)(P_0 +P_1 i)+(B_0 +B_1 i)(Q_0 +Q_1 i) \\ 
&=(A_0 P_0 +A_1 P_0 i+A_0 P_1 i-A_1 P_1 )+(B_0 Q_0 +B_1 Q_0 i+B_0 Q_1 i-B_1 
Q_1 ) \\ 
&=(A_0 P_0 +B_0 Q_0 -A_1 P_1 -B_1 Q_1 )+(A_1 P_0 +A_0 P_1 +B_1 Q_0 +B_0 Q_1 
)i
 \end{align*}
%\begin{align*}
% &(\bar {B}\bar {Q}+\bar {A}\bar {P})\\
% &=(\overline {BQ+AP} ) \\ 
% &=(A_0 P_0 +B_0 Q_0 -A_1 P_1 -B_1 Q_1 )-(A_1 P_0 +A_0 P_1 +B_1 Q_0 +B_0 Q_1)i.
% \end{align*}
This gives 
\begin{align*}
&(AP+BQ)+(\bar {B}\bar {Q}+\bar {A}\bar {P})\\
&=2Re\{AP+BQ\}\\
&=2(A_0 P_0 +B_0 Q_0 -A_1 P_1 -B_1 Q_1 )
 \end{align*}
and
\begin{align*}
 &-i(AP+BQ)+i(\bar {B}\bar {Q}+\bar {A}\bar {P})\\
 &=-i\left[(AP+BQ)-(\bar {B}\bar {Q}+\bar {A}\bar {P})\right] \\
 &=2iIm\{(AP+BQ)\}i \\
 &=-2(A_1 P_0 +A_0 P_1 +B_1 Q_0 +B_0 Q_1 ) \\ 
 \end{align*}
allowing us to write
$$
{\rm Prob}(NN)=\left(A_0 P_0 +B_0 Q_0 
-A_1 P_1 -B_1 Q_1 \right)^2
$$
$$
{\rm Prob}(FF)=(A_1 P_0 +A_0 P_1 +B_1 Q_0 +B_0 Q_1 )^2
$$
Also, 
\begin{align*}
&(-A\bar {Q}+B\bar {P})\\
&=(-A_0 -A_1 i)(Q_0 -Q_1 i)+(B_0 +B_1 i)(P_0 -P_1 i) \\ 
&=(-A_0 Q_0 -A_1 Q_0 i+A_0 Q_1 i-A_1 Q_1 )+(B_0 P_0 +B_1 P_0 i-B_0 P_1 i+B_1 
P_1 ) \\ 
&=(B_0 P_0 +B_1 P_1 -A_0 Q_0 -A_1 Q_1 )+(B_1 P_0 +A_0 Q_1 -B_0 P_1 -A_1 Q_0 
)i 
\end{align*}
%and
%\begin{align*} 
%&(-\bar {B}P+\bar {A}Q)\\
%&=-(\overline {-A\bar {Q}+B\bar {P}} ) \\ 
% &=-\left[ {(B_0 P_0 +B_1 P_1 -A_0 Q_0 -A_1 Q_1 )-(B_1 P_0 +A_0 Q_1 -B_0 P_1 
%-A_1 Q_0 )i} \right] \\ 
% &=-(B_0 P_0 +B_1 P_1 -A_0 Q_0 -A_1 Q_1 )+(B_1 P_0 +A_0 Q_1 -B_0 P_1 -A_1 Q_0 
%)i
%\end{align*}
Therefore,
\begin{align*} 
 &-\eta (-A\bar {Q}+B\bar {P})+\bar {\eta }(-\bar {B}P+\bar {A}Q) \\
 &=-\eta (-A\bar {Q}+B\bar {P})-\bar {\eta }(\overline {-A\bar {Q}+B\bar {P}} ) \\ 
 &=-\left[ {\eta (-A\bar {Q}+B\bar {P})+(\overline {\eta (-A\bar {Q}+B\bar{P}} )} \right] \\
&=-2Re\{\eta (-A\bar {Q}+B\bar {P})\} \\ 
 &=-\frac{2}{\sqrt 2}(B_0 P_0 +B_1 P_1 -A_0 Q_0 -A_1 Q_1 )-(B_1 P_0 +A_0 Q_1 -B_0 P_1 -A_1 Q_0) 
% &=Re\{(-A\bar {Q}+B\bar {P})\}-Im\{(-A\bar {Q}+B\bar {P})\} 
\end{align*}
and
\begin{align*} 
&\bar {\eta }(-A\bar {Q}+B\bar {P})-\eta (-\bar {B}P+\bar {A}Q) \\
&=\bar {\eta}(-A\bar {Q}+B\bar {P})-\eta (\overline {-A\bar {Q}+B\bar {P}} ) \\ 
 &=-i\left[ {\eta (-A\bar {Q}+B\bar {P})-\overline {(\eta (-A\bar {Q}+B\bar{P}} )} \right]\\
&=-2Im\{\eta (-A\bar {Q}+B\bar {P})\} \\ 
&=-\frac{2}{\sqrt 2}(B_0 P_0 +B_1 P_1 -A_0 Q_0 -A_1 Q_1 )+(B_1 P_0 +A_0 Q_1 -B_0 P_1 -A_1 Q_0 ) \\ 
%&=Re\{(-A\bar {Q}+B\bar {P})\}+Im\{(-A\bar {Q}+B\bar {P})\} 
\end{align*}
allowing us to write
$$
{\rm Prob}(NF)=\frac{1}{2}(B_0 P_0 +B_1 P_1 -A_0 Q_0 -A_1 Q_1 )-(B_1 P_0 +A_0 Q_1 -B_0 P_1 -A_1 Q_0)^2
$$
$$
{\rm Prob}(FN)=\frac{1}{ 2}(B_0 P_0 +B_1 P_1 -A_0 Q_0 -A_1 Q_1 )+(B_1 P_0 +A_0 Q_1 -B_0 P_1 -A_1 Q_0 )^2
$$
 
\section{Quaternionic Coordinatization of the Payoff Function}

Now make the following identification between elements of $SU(2)$ and $Sp(1)$: 
$$
\left( {{\begin{array}{*{20}c}
 A \hfill & B \hfill \\
 {-\bar {B}} \hfill & {\bar {A}} \hfill \\
\end{array} }} \right) \longleftrightarrow p=A+B\eta j
$$
and
$$
\left( {{\begin{array}{*{20}c}
 P \hfill & {-\bar {Q}} \hfill \\
 Q \hfill & {\bar {P}} \hfill \\
\end{array} }} \right) \longleftrightarrow q=P-\eta jQ
$$ 
Then
\begin{align*} 
pq&=(A+B\eta j)(P-\eta jQ)=AP+B\eta jP-A\eta jQ-B\eta j\eta jQ \\ 
&=AP+\eta B\bar {P}j-\eta A\bar {Q}j-\eta B\bar {\eta }j^2Q\mbox{ } \\ 
&=AP+\eta B\bar {P}j-\eta A\bar {Q}j+\eta B\bar {\eta }Q \\ 
&=AP+\eta B\bar {P}j-\eta A\bar {Q}j+BQ \\ 
& =\left( {AP+BQ} \right)+\eta (B\bar {P}j-A\bar {Q}j) \\ 
& =\left( {AP+BQ} \right)+\eta (B\bar {P}-A\bar {Q})j \\ 
& =\left( {AP+BQ} \right)+(B\bar {P}-A\bar {Q})\eta j \\ 
&=\left( {AP+BQ} \right)+(-A\bar {Q}+B\bar {P})\eta j
\end{align*}
Expanding with respect to the complex numbers $A$, $B$, $P$, and $Q$ gives,
\begin{align*}
&=\left[ {(A_0 +A_1 i)(P_0 +P_1 i)+(B_0 +B_1 i)(Q_0 +Q_1 i)} \right]\\
&+\left[ {(-A_0 -A_1 i)(Q_0 -Q_1 i)+(B_0 +B_1 i)(P_0 -P_1 i)} \right]\eta j 
\end{align*}
\begin{align*}
&=(A_0 P_0 +A_1 P_0 i+A_0 P_1 i-A_1 P_1 )\\
&+(B_0 Q_0 +B_1 Q_0 i+B_0 Q_1 i-B_1 Q_1 )\\
&+(-A_0 Q_0 -A_1 Q_0 i+A_0 Q_1 i-A_1 Q_1 )\eta j \\
&+(B_0 P_0 +B_1 P_0 i-B_0 P_1 i+B_1 P_1 )\eta j
\end{align*}
\begin{align*}
&=A_0 P_0 +B_0 Q_0 -A_1 P_1 -B_1 Q_1 +A_1 P_0 i \\
&+A_0 P_1 i+B_1 Q_0 i+B_0 Q_1 i-A_0 Q_0 \eta j +B_0 P_0 \eta j \\
&+B_1 P_1 \eta j-A_1 Q_1 \eta j -A_1 Q_0 \eta ij+A_0 Q_1 \eta ij+B_1 P_0 \eta ij-B_0 P\eta _1 ij
\end{align*}
\begin{align*}
& =(A_0 P_0 +B_0 Q_0 -A_1 P_1 -B_1 Q_1 )+(A_1 P_0 +A_0 P_1 +B_1 Q_0 +B_0 Q_1 )i \\
&+(-A_0 Q_0 +B_0 P_0 +B_1 P_1 -A_1 Q_1 )\eta j\mbox{ }+\mbox{(}-A_1 Q_0 +A_0 Q_1 +B_1 P_0 -B_0 P_1 )\eta k \\ \\ 
&=(A_0 P_0 +B_0 Q_0 -A_1 P_1 -B_1 Q_1 )+(A_1 P_0 +A_0 P_1 +B_1 Q_0 +B_0 Q_1)i\\
&+(-A_0 Q_0 +B_0 P_0 +B_1 P_1 -A_1 Q_1 )(1+i)j \\
&+(-A_1 Q_0 +A_0 Q_1 +B_1 P_0 -B_0 P_1 )(1+i)k
\end{align*}
\begin{align*}
&=(A_0 P_0 +B_0 Q_0 -A_1 P_1 -B_1 Q_1 )+(A_1 P_0 +A_0 P_1 +B_1 Q_0 +B_0 Q_1)i \\
&+(-A_0 Q_0 +B_0 P_0 +B_1 P_1 -A_1 Q_1 )j +(-A_0 Q_0 +B_0 P_0 +B_1 P_1 -A_1 Q_1 )ij \\
&+(-A_1 Q_0 +A_0 Q_1 +B_1 P_0 -B_0 P_1 )k+(-A_1 Q_0 +A_0 Q_1 +B_1 P_0 -B_0 P_1 )ik 
\end{align*}
\begin{align*}
&=(A_0 P_0 +B_0 Q_0 -A_1 P_1 -B_1 Q_1 )+(A_1 P_0 +A_0 P_1 +B_1 Q_0 +B_0 Q_1 )i\\
&+(-A_0 Q_0 +B_0 P_0 +B_1 P_1 -A_1 Q_1 )j+(-A_0 Q_0 +B_0 P_0 +B_1 P_1 -A_1 Q_1 )k\\
&+(-A_1 Q_0 +A_0 Q_1 +B_1 P_0 -B_0 P_1 )k-(-A_1 Q_0 +A_0 Q_1 +B_1 P_0 -B_0 P_1 )j
\end{align*}
\begin{align*}
&=(A_0 P_0 +B_0 Q_0 -A_1 P_1 -B_1 Q_1 )+(A_1 P_0 +A_0 P_1 +B_1 Q_0 +B_0 Q_1)i \\
&+(-A_0 Q_0 +B_0 P_0 +B_1 P_1 -A_1 Q_1 )j-(-A_1 Q_0 +A_0 Q_1 +B_1 P_0 -B_0 P_1 )j \\ 
&+(-A_0 Q_0 +B_0 P_0 +B_1 P_1 -A_1 Q_1 )k+(-A_1 Q_0 +A_0 Q_1 +B_1 P_0 -B_0 P_1 )k
\end{align*}
\begin{align*}
&=(A_0 P_0 +B_0 Q_0 -A_1 P_1 -B_1 Q_1 )+(A_1 P_0 +A_0 P_1 +B_1 Q_0 +B_0 Q_1)i \\ 
&+\left[ {(-A_0 Q_0 +B_0 P_0 +B_1 P_1 -A_1 Q_1 )-(-A_1 Q_0 +A_0 Q_1 +B_1 P_0 -B_0 P_1 )} \right]j \\ 
&+\left[ {(-A_0 Q_0 +B_0 P_0 +B_1 P_1 -A_1 Q_1 )+(-A_1 Q_0 +A_0 Q_1 +B_1 P_0 -B_0 P_1 )} \right]k 
\end{align*}
Set
$$
\pi _1 \mbox{(}pq\mbox{)}=(A_0 P_0 +B_0 Q_0 -A_1 P_1 -B_1 Q_1 )
$$
$$
\pi _2 \mbox{(}pq\mbox{)}=(A_1 P_0 +A_0 P_1 +B_1 Q_0 +B_0 Q_1 )
$$
$$
 \pi _3 \mbox{(}pq\mbox{)}=(-A_0 Q_0 +B_0 P_0 +B_1 P_1 -A_1 Q_1 )-\mbox{(}-A_1 Q_0 +A_0 Q_1 +B_1 P_0 
-B_0 P_1 )
$$
$$
 \pi _4 \mbox{(}pq\mbox{)}=(-A_0 Q_0 +B_0 P_0 +B_1 P_1 -A_1 Q_1 )\mbox{ }+\mbox{(}-A_1 Q_0 +A_0 Q_1 
+B_1 P_0 -B_0 P_1 )
$$
Then
\[
\begin{array}{l}
 {\rm prob}(NN)=\pi _1 (pq)^2 \\ 
 \\ 
{\rm prob}(NF)=\pi _4 (pq)^2 \\ 
 \\ 
{\rm prob}(FN)=\pi _3 (pq)^2 \\ 
 \\ 
{\rm prob}(FF)=\pi _2 (pq)^2 \\ 
 \end{array}
\]
%\end{document}


==> Chapter5.tex <==
% Converted from Microsoft Word to LaTeX
%% by Chikrii Softlab Word2TeX converter (version 3.0)
%% Copyright (C) 1999-2003 Chikrii Softlab. All rights reserved.
%% http://www.chikrii.com
%% mailto: info@chikrii.com
%% License: CSL#0036C0
%
%\documentclass[12pt]{article}
%\usepackage{latexsym}
%\usepackage{amssymb}
%\usepackage{amsmath}
%\usepackage{graphicx}
%\usepackage{longtable}
% \usepackage{setspace}
% \usepackage{amsthm}
%\doublespacing
%\newtheorem{theorem}{Theorem}
%\newtheorem{definition}{Definition}
%\newtheorem{corollary}{Corollary}
%\begin{document}

\chapter{Octonionic Co-ordinatization of 3 Player, 2 Strategy Quantum Games}
%%\author{Aden Ahmed, Steve Bleiler, Faisal Shah Khan}
%\maketitle
%
%\begin{abstract}
%We develop an octonionic representation of the payoff function for a three player, two strategy, maximally entangled quantum game.
%\end{abstract}

%\section{Introduction}\label{intro}

We wish to obtain a computational framework similar to that of Landsburg's, discussed in chapter 4, for three player, two strategy maximally entangled quantum games. To this end, we develop an octonionic computational framework that constructs maps analogous to the maps $L$ and $L_{*}$ of Figure \ref{L map}. Our game will be quantized in a manner similar to that given by Eisert et al \cite{Eisert}.

We consider a three player game where each player has access to exactly two 
pure strategies. Each player communicates his strategic choice to a referee via 
a qubit in superposition. The referee initially sends to the three players 
qubits in the maximally entangled state $\left| {000} \right\rangle +\left| 
{111} \right\rangle $. The two classical pure strategies available to the 
players are \textit{flip} denoted by $F$, and \textit{no flip} denoted by $N$, represented respectively by 
the $SU(2)$ matrices
\[
F=\left( {{\begin{array}{*{20}c}
 0 \hfill & \eta \hfill \\
 {-\bar {\eta }} \hfill & 0 \hfill \\
\end{array} }} \right),\mbox{ } 
N=\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill \\
 0 \hfill & 1 \hfill \\
\end{array} }} \right)
\]
where $\eta \in U(1)$ is chosen such that the eight outcome states of our 
three player game form an orthogonal basis of the state 
space $\mathbb{C}^8$ with the {\it observation} basis 
$$
\mathcal{B}=\left\{ {\left| {000} \right\rangle 
,\left| {001} \right\rangle ,\left| {010} \right\rangle ,\left| {011} 
\right\rangle ,\left| {100} \right\rangle ,\left| {101} \right\rangle 
,\left| {110} \right\rangle ,\left| {111} \right\rangle } \right\}.
$$
These eight outcome states are denoted by 
$$
\mathcal{B}_{FN}=\left\{NNN, NNF, NFN, NFF, FNN, FNF, FFN, FFF\right\}
$$
where any of these 
triples of $N $and $F$ represent the pure strategy choices of the players I and II 
and III, respectively. Now a direct calculation shows that $\eta ^6=1$, so 
setting 
$$
\eta =\frac{1}{2}+\frac{\sqrt 3 }{2}i
$$ 
makes the eight states in in $\mathcal{B}_{FN}$ orthogonal.
%
%A pure quantum strategy for each player can be represented by a matrix 
%in $SU(2)\cong S^3\cong SP(1)$, the group of unit quaternions. This gives a quaternionic co-ordinatization of the game. Indeed, Landsburg gives just such a {\it quaternionization} of two player, two strategy, maximally entangled quantum games in [ ]. As in our 
%case, each player in [ Lands] communicates his strategic choice to a referee via a 
%qubit in superposition. The referee initially sends to the two players qubits 
%in the maximally entangled state $\left| {00} \right\rangle +\left| {11} 
%\right\rangle $. The two classical pure strategies available to the players 
%are \textit{flip} denoted by $F$, and \textit{no flip} denoted by $N$, represented respectively by 
%the $SU(2)$matrices
%\[
%F=\left( {{\begin{array}{*{20}c}
% 0 \hfill & \eta \hfill \\
% {-\bar {\eta }} \hfill & 0 \hfill \\
%\end{array} }} \right),\mbox{ } 
%N=\left( {{\begin{array}{*{20}c}
% 1 \hfill & 0 \hfill \\
% 0 \hfill & 1 \hfill \\
%\end{array} }} \right)
%\]
%where $\eta \in U(1)$ is chosen such that the four outcome states of our two 
%player game formed an orthogonal basis of the state space $\mathbb{C}^4$ with 
%standard basis 
%$$
%\left\{ {\left| {00} \right\rangle ,\left| {01} \right\rangle 
%,\left| {10} \right\rangle ,\left| {11} \right\rangle } \right\}.
%$$
%These four outcome states are denoted by 
%$$
%\left\{NN, NF, FN, FF \right\}
%$$
%where any of these pairs of $N$ and $F$ represent the pure strategy choices of the players I and II respectively. 
%A direct calculation in this case shows that $\eta ^8=1$, so setting
%$$
%\eta 
%=\frac{1+i}{\sqrt 2 }
%$$ 
%makes the four states \textit{NN}, \textit{NF}, \textit{FN}, \textit{FF} orthogonal. In both our game and Landsburg's  game, a pure quantum strategy for each player now 
%corresponds to a general element of $SU(2)$ acting on a player's qubit before 
%the player sends it to the referee. A classical pure strategy corresponds to 
%the player's choice of one of the matrices $F$ or $N$ given above for these 
%actions on their qubits.
%
%Either taking a mixture, a superposition, or a mixed superposition of the 
%pure strategies produces a probability distribution over the four outcomes 
%of the game. The expected value for each pair of strategic choices by the 
%players forms the set of payoffs for the game. After identifying each pure 
%quantum strategy, i.e each superposition of the classical pure strategies, 
%for each player with a suitable unit quaternion $p$ or $q$, Landsburg shows that 
%the probability distribution over the four possible outcomes when the 
%players use these strategies is then given by the squares of the 
%coefficients of the unit quaternion \textit{pq}. Note that the superpositions include 
%the mixtures. From this, Landsburg is able to obtain payoff expressions for 
%when the players use mixtures, superpositions, or mixed superpositions of 
%the pure classical strategies. Using these expressions, Landsburg can 
%classify the Nash equilibria of the maximally entangled quantum game, and 
%for zero sum games, can show that by using mixed superpositions of 
%strategies, the players can guarantee to themselves the average of the four 
%possible outcomes. Frequently, this is a superior equilibrium than that 
%available to players restricted to classical mixed strategies.
%
%We wish to extend Landsburg's results to the three player, two pure strategy 
%situations. To this end, we develop an {\it octonianization} of our maximally 
%entangled three player, two strategy quantum game describe above. We 
%identify each strategic choice of player I, II, or III with a unit octonion 
%$s$, $t$, or $u$ respectively, where each of $s$, $t$, or $u$ lies in a particular, possibly different 
%copy of the unit quaternions embedded in the octonionic real division 
%algebra. The probability distribution over our eight possible outcomes is 
%then shown to be determined by an expression involving the associated triple 
%product $(st)u$ of the strategies $s$, $t$, and $u$. The associated nature of this 
%product is in fact natural as the octonions are in general non-associative. 
%As in Landsburg's case, these identifications above and the resulting 
%probability distribution over the outcome allows us to examine the effect on 
%the payoffs to each player of the game when players use mixtures, 
%superpositions, or mixed superpositions of the pure strategies.

\section{Octonions}

The octonions $\mathbb{O}$ are a non-associative 8-dimensional, normed, real 
division algebra given as
\[
a_0 +\sum\limits_{j=1}^7 {a_j } i_j 
\]
where $a_j \in \mathbb{R}$, and the $i_j $'s have the property that $i_j 
^2=-1$. Moreover, these seven $i_j $'s (along with $i_0 $ can be used to 
form seven copies of the quaternions $\mathbb{H}$ embedded within $\mathbb{O}$
as certain triple products of the $i_1 \ldots i_7 $ are also equal to -1. A 
mnemonic for which these triple products are in fact equal to -1 is given by 
an edge oriented Fano plane. The Fano plane illustrated in Figure {\ref{Fanoplane}} indicates how 
these triple products work. In particular, when the $i_j ,i_k ,i_l $ are 
cyclically ordered as in the Fano plane
\begin{figure}[htbp]
\centerline{\includegraphics[scale=0.8]{fanoplane}}
\caption{The Fano plane.}
\label{Fanoplane}
\end{figure}
then $i_j ^2=i_k ^2=i_l ^2=i_j i_k i_l =-1$ showing that in general $i_j i_k 
=i_l =-i_k i_j $. 

We will be interested in three copies of $\mathbb{H}$ with a common embedded 
copy of the complex numbers $\mathbb{C}$. For this we choose the copies $\mathbb{H}_1$, $\mathbb{H}_2$, $\mathbb{H}_3$ of the quaternions $\mathbb{H}$ with bases 
$$\mathcal{B}_{\mathbb{H}_1}=\left\{{1,i_1 ,i_2 ,i_4 } \right\},\mbox{ }\mathcal{B}_{\mathbb{H}_2}=\left\{ {1,i_1 ,i_5 ,i_6 } 
\right\},\,\mathcal{B}_{\mathbb{H}_3}=\left\{ {1,i_1 ,i_3 ,i_7 } \right\}
$$ 
respectively. We focus our 
attention on the unit $S^3$'s in each of these four dimensional copies of 
$\mathbb{H}$ and consider each such $S^3$ as a ``longitude'' of the unit 
octonions which form a seven dimensional sphere $S^7 \subset \mathbb{O}$.

\section{Octonionic Representation of Three Player, Two Strategy 
Quantum Games}

We now identify the pure quantum strategies available to each player with a 
particular unit octonion. Discounting phase, these quantum strategies each 
correspond to an element of $SU(2)$ as indicated for example in the appendix 
of [landsburg].

Recall that the elements of the group $SU(2)$ are $2\times 2$ complex matrices 
with determinant one, and can be written in the form
\[
\left( {{\begin{array}{*{20}c}
 x \hfill & y \hfill \\
 {-\bar {y}} \hfill & {\bar {x}} \hfill \\
\end{array} }} \right)
\]
If player 1 chooses the pure quantum strategy corresponding to
$$
\mathbb{A}=\left( 
{{\begin{array}{*{20}c}
 A \hfill & B \hfill \\
 {-\bar {B}} \hfill & {\bar {A}} \hfill \\
\end{array} }} \right)
$$
where $A=a_0 +a_1 i$, $B=b_0 +b_1 i$, identify this 
strategy with the unit octonion given by 
\[
\begin{array}{l}
 s_{00} \equiv A+B\bar {\eta }i_4 =a_0 +a_1 i_1 +\left( {b_0 +b_1 i_1 } 
\right)\left( {\frac{1}{2}-\frac{\sqrt 3 }{2}i_1 } \right)i_4 \\ 
 \;\;\;\;\;=a_0 +a_1 i_1 +\left( {\frac{\sqrt 3 }{2}b_0 -\frac{1}{2}b_1 } 
\right)i_2 +\left( {\frac{1}{2}b_0 +\frac{\sqrt 3 }{2}b_1 } \right)i_4 \\ 
 \end{array}
\]
The subscript of $s$ is used to track sign changes on the two real 
coefficients in the expression for $s$, namely,$a_0 ,a_1 $. A positive sign 
will be represented by 0 and a sign change to a negative in the expression 
for $s$ will be represented by 1. This notation will be used below to extract 
the appropriate coefficient for the desired probability distribution.

Similarly, if player 2 chooses a quantum strategy corresponding to
$$
\mathbb{P}=\left( 
{{\begin{array}{*{20}c}
 P \hfill & Q \hfill \\
 {-\bar {P}} \hfill & {\bar {Q}} \hfill \\
\end{array} }} \right)
$$
where $P=p_0 +p_1 i$, $Q=q_0 +q_1 i$, consider the 
unit octonion give by
\[
\begin{array}{l}
 t_{00} \equiv P+Q\bar {\eta }i_6 =p_0 +p_1 i_1 +\left( {q_0 +q_1 i_1 } 
\right)\left( {\frac{1}{2}-\frac{\sqrt 3 }{2}i_1 } \right)i_6 \\ 
 \;\;\;\;=p_0 +p_1 i_1 +\left( {\frac{\sqrt 3 }{2}q_0 -\frac{1}{2}q_1 } 
\right)i_5 +\left( {\frac{1}{2}q_0 +\frac{\sqrt 3 }{2}q_1 } \right)i_6 \\ 
 \end{array}
\]
And if player 3 chooses the quantum strategy corresponding to
$$
\mathbb{E}=\left( 
{{\begin{array}{*{20}c}
 E \hfill & F \hfill \\
 {-\bar {F}} \hfill & {\bar {E}} \hfill \\
\end{array} }} \right)
$$
where $E=e_0 +e_1 i$, $F=f_0 +f_1 i$, consider the 
unit octonion given by
\[
\begin{array}{l}
 u_{00} \equiv E+F\bar {\eta }i_7 =e_0 +e_1 i_1 +\left( {f_0 +f_1 i_1 } 
\right)\left( {\frac{1}{2}-\frac{\sqrt 3 }{2}i_1 } \right)i_7 \\ 
 \;\;\;\;\;=e_0 +e_1 i_1 +\left( {\frac{\sqrt 3 }{2}f_0 -\frac{1}{2}f_1 } 
\right)i_3 +\left( {\frac{1}{2}f_0 +\frac{\sqrt 3 }{2}f_1 } \right)i_7 \\ 
 \end{array}
\]

\begin{theorem}\label{theorem}{\rm 
If in the maximally entangled three players, two strategy quantum game, 
player 1 plays the pure quantum strategy $\mathbb{A}$, player 2 the pure quantum strategy $\mathbb{P}$, and player 3 the pure quantum strategy $\mathbb{E}$, then the probability distribution over the set of outcomes $\mathcal{B}_{FN}$ is given by }
\[
\begin{array}{l}
 pr(NNN)=\left[ {\pi _0 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} 
+\left( {s_{01} t_{10} } \right)u_{01} }{2}} \right)} \right]^2+\left[ {\pi 
_0 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} -\left( {s_{01} 
t_{10} } \right)u_{01} }{2}} \right)} \right]^2 \\ 
 pr(FFF)=\left[ {\pi _1 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} 
+\left( {s_{01} t_{10} } \right)u_{01} }{2}} \right)} \right]^2+\left[ {\pi 
_1 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} -\left( {s_{01} 
t_{10} } \right)u_{01} }{2}} \right)} \right]^2 \\ 
 pr(FFN)=\left[ {\pi _3 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} 
+\left( {s_{01} t_{10} } \right)u_{01} }{2}} \right)} \right]^2+\left[ {\pi 
_3 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} -\left( {s_{01} 
t_{10} } \right)u_{01} }{2}} \right)} \right]^2 \\ 
 pr(NNF)=\left[ {\pi _7 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} 
+\left( {s_{01} t_{10} } \right)u_{01} }{2}} \right)} \right]^2+\left[ {\pi 
_7 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} -\left( {s_{01} 
t_{10} } \right)u_{01} }{2}} \right)} \right]^2 \\ 
 pr(NFF)=\left[ {\pi _2 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} 
+\left( {s_{01} t_{00} } \right)u_{00} }{2}} \right)} \right]^2+\left[ {\pi 
_2 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} -\left( {s_{01} 
t_{00} } \right)u_{00} }{2}} \right)} \right]^2 \\ 
 pr(FNN)=\left[ {\pi _4 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} 
+\left( {s_{01} t_{00} } \right)u_{00} }{2}} \right)} \right]^2+\left[ {\pi 
_4 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} -\left( {s_{01} 
t_{00} } \right)u_{00} }{2}} \right)} \right]^2 \\ 
 pr(FNF)=\left[ {\pi _5 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} 
+\left( {s_{01} t_{00} } \right)u_{00} }{2}} \right)} \right]^2+\left[ {\pi 
_5 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} -\left( {s_{01} 
t_{00} } \right)u_{00} }{2}} \right)} \right]^2 \\ 
 pr(NFN)=\left[ {\pi _6 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} 
+\left( {s_{01} t_{00} } \right)u_{00} }{2}} \right)} \right]^2+\left[ {\pi 
_6 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} -\left( {s_{01} 
t_{00} } \right)u_{00} }{2}} \right)} \right]^2 \\ 
 \end{array}
\]
\end{theorem}
The proof of theorem \ref{theorem} is technical, and is based on the ideas developed in the following sections.

\subsection{The Game State}

Let
$$
\left\{\left|0\right\rangle=\left( {{\begin{array}{*{20}c}
 1 \hfill \\
 0 \hfill \\
\end{array} }} \right), \hspace{.05in}
\left|1\right\rangle=\left( {{\begin{array}{*{20}c}
 0 \hfill \\
 1 \hfill \\
\end{array} }} \right)\right\}
$$
be the {\it observation} basis of for the state space $\mathbb{C}^2$ of a qubit, often referred to as the computational basis in quantum computation literature. The observational basis for the state space $\mathbb{C}^8$ of three qubits $\mathcal{B}$ in section \ref{intro} is got from the tensor product of three copies of $\mathbb{C}^2$. With respect to the basis $\mathcal{B}$, consider three qubits in the initial state
$$
\frac{1}{\sqrt 2 }\left( 
{\left|0\right\rangle \otimes \left|0\right\rangle \otimes \left|0\right\rangle + \left|1\right\rangle \otimes \left|1\right\rangle \otimes \left|1\right\rangle} \right).
$$
Player 1 acts on 
the first qubit via $\mathbb{A}$, player 2 acts on the second qubit via $\mathbb{P}$, and player 3 acts on the third qubit via $\mathbb{E}$, respectively. After the players act on the appropriate qubits (and after ignoring the normalization constant$1/\sqrt 2 $), our initial state 
becomes
\[
\left( \begin{array}{*{20}c}
 A \hfill \\
 -\bar {B} \hfill \\
\end{array} \right) \otimes \left( \begin{array}{*{20}c}
 P \hfill \\
 -\bar {Q} \hfill \\
\end{array}  \right)\otimes \left( \begin{array}{*{20}c}
 E \hfill \\
 -\bar {F} \hfill \\
\end{array} \right)+\left( \begin{array}{*{20}c}
 B \hfill \\
 \bar {A} \hfill \\
\end{array}  \right)\otimes \left( \begin{array}{*{20}c}
 Q \hfill \\
 \bar {P} \hfill \\
\end{array}  \right)\otimes \left( \begin{array}{*{20}c}
 F \hfill \\
 \bar {E} \hfill \\
\end{array}  \right)
\]
Expanding using the bilinearity of the tensor product and collecting the coefficients over the elements of the basis $\mathcal{B}$ we obtain
%\[
%\left( {A H-\bar{B} T} \right)\otimes \left( {PH-\bar 
%{Q} T} \right)\otimes \left( {E H-\bar {F} T} \right)+\left( 
%{B H+\bar {A} T} \right)\otimes \left( {Q H+\bar {P} T} 
%\right)\otimes \left( {F H+\bar{E} T} \right)
%\]
\begin{align*}
&\left(APE+BQF\right)\left(\left|0\right\rangle \otimes \left|0\right\rangle \otimes \left|0\right\rangle \right)+ \left(BQ\bar{E}-AP\bar{F} 
\right)\left(\left|0\right\rangle \otimes \left|0\right\rangle \otimes \left|1\right\rangle \right)\\
&+\left(B\bar{P}F-A\bar{Q}E \right)\left(\left|0\right\rangle \otimes 
\left|1\right\rangle \otimes \left|0\right\rangle\right) +\left( A\bar{Q}\bar{F}+B\bar{P}\bar{E}\right) \left(\left|0\right\rangle \otimes 
\left|1\right\rangle \otimes \left|1\right\rangle \right) \\ 
&+\left( \bar{A}QF-\bar{B}PE \right) \left(\left|1\right\rangle \otimes \left|0\right\rangle \otimes \left|0\right\rangle \right)+\left( \bar 
{B}P\bar {F}+\bar {A}Q\bar {E} \right) \left(\left|1\right\rangle \otimes \left|0\right\rangle \otimes \left|1\right\rangle \right) \\
&+\left( \bar {B}\bar {Q}E+\bar {A}\bar {P}F \right) \left( \left|1\right\rangle \otimes \left|1\right\rangle \otimes \left|0\right\rangle \right)+\left( \bar 
{A}\bar {P}\bar {E}-\bar {B}\bar {Q}\bar {F} \right)\left(\left|1\right\rangle \otimes \left|1\right\rangle \otimes \left|1\right\rangle \right)
\end{align*}
As a vector in $\mathbb{C}^8$ this is
\begin{equation}\label{vect in C8}
\left( 
{{\begin{array}{*{20}c}
 {APE+BQF} \hfill \\
 {BQ\bar {E}-AP\bar {F}} \hfill \\
 {B\bar {P}F-A\bar {Q}E} \hfill \\
 {A\bar {Q}\bar {F}+B\bar {P}\bar {E}} \hfill \\
 {\bar {A}QF-\bar {B}PE} \hfill \\
 {\bar {B}P\bar {F}+\bar {A}Q\bar {E}} \hfill \\
 {\bar {B}\bar {Q}E+\bar {A}\bar {P}F} \hfill \\
 {\bar {A}\bar {P}\bar {E}-\bar {B}\bar {Q}\bar {F}} \hfill \\
\end{array} }} \right)%{\begin{array}{*{20}c}
% {HHH} \hfill \\
% {HHT} \hfill \\
% {HTH} \hfill \\
% {HTT} \hfill \\
% {THH} \hfill \\
% {THT} \hfill \\
% {TTH} \hfill \\
% {TTT} \hfill \\
%\end{array} } \\ 
% \end{array}
\end{equation}
Call the vector in (\ref{vect in C8})the \textit{game state}.

\subsection{Orthogonality and Change of Basis}
Recall from section \ref{intro} that the action \textit{no flip} is represented by the $SU(2)$ matrix 
$$
N=\left( 
{{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill \\
 0 \hfill & 1 \hfill \\
\end{array} }} \right)
$$ 
and the action \textit{flip} by 
$$
F=\left( {{\begin{array}{*{20}c}
 0 \hfill & \eta \hfill \\
 {-\bar {\eta }} \hfill & 0 \hfill \\
\end{array} }} \right).
$$ 
Note that $F\left|0\right\rangle=-\bar{\eta }\left|1\right\rangle$ and $F\left|1\right\rangle=\eta\left|0\right\rangle$, where $\eta $ is a unit complex number to be determined shortly. In section \ref{intro} we set the outcome states of the game to be the set 
$$
\mathcal{B}_{FN}=\left\{NNN, NNF, NFN, NFF, FNN, FNF, FFN, FFF\right\}
$$
which is to serve as an orthogonal basis for $\mathbb{C}^8$. Call this the {\it action basis}. For each element of the action basis, the corresponding values of $A$,$ B$,$ P$,$ Q$,$ E$, $F$ is given in the table below.
\begin{longtable}[htbp]
{|p{17pt}|l|p{10pt}|l|p{10pt}|l|p{10pt}|}
\hline
\endhead
\hline
\endfoot
& 
$A$& 
$B$& 
$P$& 
$Q$& 
$E$& 
$F$ \\
\hline
\textit{NNN}& 
1& 
0& 
1& 
0& 
1& 
0 \\
\hline
\textit{NNF}& 
1& 
0& 
1& 
0& 
0& 
$\eta $ \\
\hline
\textit{NFN}& 
1& 
0& 
0& 
$\eta $& 
1& 
0 \\
\hline
\textit{NFF}& 
1& 
0& 
0& 
$\eta $& 
0& 
$\eta $ \\
\hline
\textit{FNN}& 
0& 
$\eta $& 
1& 
0& 
1& 
0 \\
\hline
\textit{FNF}& 
0& 
$\eta $& 
1& 
0& 
0& 
$\eta $ \\
\hline
\textit{FFN}& 
0& 
$\eta $& 
0& 
$\eta $& 
1& 
0 \\
\hline
\textit{FFF}& 
0& 
$\eta $& 
0& 
$\eta $& 
0& 
$\eta $
\label{tab1}
\end{longtable}
Plugging these values of the $A$,$ B$,$ P$,$ Q$,$ E$, $F$ into the game state gives the following relationship between the observational basis $\mathcal{B}$ and the action basis $\mathcal{B}_{FN}$.
\[
NNN=\left( {{\begin{array}{*{20}c}
 1 \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 1 \hfill \\
\end{array} }} \right),
\quad
NNF=\left( {{\begin{array}{*{20}c}
 0 \hfill \\
 {-\bar {\eta }} \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 \eta \hfill \\
 0 \hfill \\
\end{array} }} \right),
\quad
NFN=\left( {{\begin{array}{*{20}c}
 0 \hfill \\
 0 \hfill \\
 {-\bar {\eta }} \hfill \\
 0 \hfill \\
 0 \hfill \\
 \eta \hfill \\
 0 \hfill \\
 0 \hfill \\
\end{array} }} \right),
\quad
NFF=\left( {{\begin{array}{*{20}c}
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 {\bar {\eta }^2} \hfill \\
 {\eta ^2} \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
\end{array} }} \right),
\]
\[
FFF=\left( {{\begin{array}{*{20}c}
 {\eta ^3} \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 {-\bar {\eta }^3} \hfill \\
\end{array} }} \right),
\quad
FFN=\left( {{\begin{array}{*{20}c}
 0 \hfill \\
 {\eta ^2} \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 {\bar {\eta }^2} \hfill \\
 0 \hfill \\
\end{array} }} \right),
\quad
FNN=\left( {{\begin{array}{*{20}c}
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
 \eta \hfill \\
 {-\bar {\eta }} \hfill \\
 0 \hfill \\
 0 \hfill \\
 0 \hfill \\
\end{array} }} \right),
\quad
FNF=\left( {{\begin{array}{*{20}c}
 0 \hfill \\
 0 \hfill \\
 \eta^2 \hfill \\
 0 \hfill \\
 0 \hfill \\
 \bar{\eta}^2 \hfill \\
 0 \hfill \\
 0 \hfill \\
\end{array} }} \right)
\]
The value of $\eta$ that ensure the orthogonality of $\mathcal{B}_{FN}$ is computed from the 
non-trivial orthogonality conditions.
\[
\left\langle {NNN,FFF} \right\rangle =\bar {\eta }^3-\eta ^3=0,
\]
\[
\left\langle {NNF,FFN} \right\rangle =-\bar {\eta }\cdot \bar {\eta }^2+\eta 
\cdot \eta ^2=-\bar {\eta }^3+\eta ^3=0,
\]
\[
\left\langle {NFN,FNF} \right\rangle =-\bar {\eta }\cdot \bar {\eta }^2+\eta 
\cdot \eta ^2=-\bar {\eta }^3+\eta ^3=0,
\]
\[
\left\langle {NFF,FNN} \right\rangle =\bar {\eta }^2\cdot \bar {\eta }+\eta 
^2\cdot (-\eta )=\bar {\eta }^3-\eta ^3=0
\]
Therefore $\eta ^6=1$ and $\eta =\frac{1}{2}+\frac{\sqrt 3 
}{2}i$.

The change of basis matrix of that takes the action basis to the 
observational basis is 
\[
A=\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill 
& {\eta ^3} \hfill \\
 0 \hfill & {-\bar {\eta }} \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 
\hfill & {\eta ^2} \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & {-\bar {\eta }} \hfill & 0 \hfill & 0 \hfill & {\eta 
^2} \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & {\bar {\eta }^2} \hfill & \eta \hfill & 0 
\hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & {\eta ^2} \hfill & {-\bar {\eta }} \hfill 
& 0 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & \eta \hfill & 0 \hfill & 0 \hfill & {\bar {\eta }^2} 
\hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & \eta \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & {\bar 
{\eta }^2} \hfill & 0 \hfill \\
 1 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill 
& {-\bar {\eta }^3} \hfill \\
\end{array} }} \right).
\]
This matrix is unitary (up to normalization) by construction so $\bar 
{A}^T=A^{-1}$, allowing us to easily compute the basis change matrix from the 
observational basis to the action basis to be
\[
A^{-1}=\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill 
& 1 \hfill \\
 0 \hfill & {-\eta } \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 
{\bar {\eta }} \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & {-\eta } \hfill & 0 \hfill & 0 \hfill & {\bar {\eta 
}} \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & {\eta ^2} \hfill & {\bar {\eta }^2} \hfill 
& 0 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & {\bar {\eta }} \hfill & {-\eta } \hfill & 
0 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & {\bar {\eta }^2} \hfill & 0 \hfill & 0 \hfill & {\eta 
^2} \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & {\bar {\eta }^2} \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 
\hfill & {\eta ^2} \hfill & 0 \hfill \\
 {\bar {\eta }^3} \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 
\hfill & 0 \hfill & {-\eta ^3} \hfill \\
\end{array} }} \right).
\]
By multiplying the game state in (\ref{vect in C8}) with $A^{-1}$ allows us to write the game state in the action basis.
\[
A^{-1}\left( {{\begin{array}{*{20}c}
 {APE+BQF} \hfill \\
 {BQ\bar {E}-AP\bar {F}} \hfill \\
 {B\bar {P}F-A\bar {Q}E} \hfill \\
 {A\bar {Q}\bar {F}+B\bar {P}\bar {E}} \hfill \\
 {\bar {A}QF-\bar {B}PE} \hfill \\
 {\bar {B}P\bar {F}+\bar {A}Q\bar {E}} \hfill \\
 {\bar {B}\bar {Q}E+\bar {A}\bar {P}F} \hfill \\
 {\bar {A}\bar {P}\bar {E}-\bar {B}\bar {Q}\bar {F}} \hfill \\
\end{array} }} \right)
%=&\left( {{\begin{array}{*{20}c}
% 1 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill 
%& 1 \hfill \\
% 0 \hfill & {-\eta } \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 
%{\bar {\eta }} \hfill & 0 \hfill \\
% 0 \hfill & 0 \hfill & {-\eta } \hfill & 0 \hfill & 0 \hfill & {\bar {\eta 
%}} \hfill & 0 \hfill & 0 \hfill \\
% 0 \hfill & 0 \hfill & 0 \hfill & {\eta ^2} \hfill & {\bar {\eta }^2} \hfill 
%& 0 \hfill & 0 \hfill & 0 \hfill \\
% 0 \hfill & 0 \hfill & 0 \hfill & {\bar {\eta }} \hfill & {-\eta } \hfill & 
%0 \hfill & 0 \hfill & 0 \hfill \\
% 0 \hfill & 0 \hfill & {\bar {\eta }^2} \hfill & 0 \hfill & 0 \hfill & {\eta 
%^2} \hfill & 0 \hfill & 0 \hfill \\
% 0 \hfill & {\bar {\eta }^2} \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 
%\hfill & {\eta ^2} \hfill & 0 \hfill \\
% {\bar {\eta }^3} \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 
%\hfill & 0 \hfill & {-\eta ^3} \hfill \\
%\end{array} }} \right)
%\left( {{\begin{array}{*{20}c}
% {APE+BQF} \hfill \\
% {BQ\bar {E}-AP\bar {F}} \hfill \\
% {B\bar {P}F-A\bar {Q}E} \hfill \\
% {A\bar {Q}\bar {F}+B\bar {P}\bar {E}} \hfill \\
% {\bar {A}QF-\bar {B}PE} \hfill \\
% {\bar {B}P\bar {F}+\bar {A}Q\bar {E}} \hfill \\
% {\bar {B}\bar {Q}E+\bar {A}\bar {P}F} \hfill \\
% {\bar {A}\bar {P}\bar {E}-\bar {B}\bar {Q}\bar {F}} \hfill \\
%\end{array} }} \right)
%\end{align*}
%\[
=\left( {{\begin{array}{*{20}c}
 {\left( {APE+\bar {A}\bar {P}\bar {E}} \right)+\left( {BQF-\bar {B}\bar 
{Q}\bar {F}} \right)} \hfill \\
 {\left( {\eta AP\bar {F}+\bar {\eta }\bar {A}\bar {P}F} \right)+\left( 
{-\eta BQ\bar {E}+\bar {\eta }\bar {B}\bar {Q}E} \right)} \hfill \\
 {\left( {\eta A\bar {Q}E+\bar {\eta }\bar {A}Q\bar {E}} \right)+\left( 
{-\eta B\bar {P}F+\bar {\eta }\bar {B}P\bar {F}} \right)} \hfill \\
 {\left( {\eta ^2A\bar {Q}\bar {F}+\bar {\eta }^2\bar {A}QF} \right)+\left( 
{\eta ^2B\bar {P}\bar {E}-\bar {\eta }^2\bar {B}PE} \right)} \hfill \\
 {\left( {\bar {\eta }A\bar {Q}\bar {F}-\eta \bar {A}QF} \right)+\left( 
{\bar {\eta }B\bar {P}\bar {E}+\eta \bar {B}PE} \right)} \hfill \\
 {\left( {-\bar {\eta }^2A\bar {Q}E+\eta ^2\bar {A}Q\bar {E}} \right)+\left( 
{\bar {\eta }^2B\bar {P}F+\eta ^2\bar {B}P\bar {F}} \right)} \hfill \\
 {\left( {-\bar {\eta }^2AP\bar {F}+\eta ^2\bar {A}\bar {P}F} \right)+\left( 
{\bar {\eta }^2BQ\bar {E}+\eta ^2\bar {B}\bar {Q}E} \right)} \hfill \\
 {\left( {\bar {\eta }^3APE-\eta ^3\bar {A}\bar {P}\bar {E}} \right)+\left( 
{\bar {\eta }^3BQF+\eta ^3\bar {B}\bar {Q}\bar {F}} \right)} \hfill \\
\end{array} }} \right)
%{\begin{array}{*{20}c}
% {NNN} \hfill \\
% {NNF} \hfill \\
% {NFN} \hfill \\
% {NFF} \hfill \\
% {FNN} \hfill \\
% {FNF} \hfill \\
% {FFN} \hfill \\
% {FFF} \hfill \\
%\end{array} }
\]
Note that $\eta =\frac{1}{2}+\frac{\sqrt 3 }{2}i=e^{\frac{\pi }{3}i}$ 
implies that 
$$
\eta ^2=-\bar {\eta },\;\;\;\bar {\eta }^2=-\eta ,\;\;\;and\;\eta 
^3=\bar {\eta }^3=-1.
$$
Using these equations, we simplify the expression for the game state vector with respect to the action basis and get
\[
%\left( {{\begin{array}{*{20}c}
% {\left( {APE+\bar {A}\bar {P}\bar {E}} \right)+\left( {BQF-\bar {B}\bar 
%{Q}\bar {F}} \right)} \hfill \\
% {\left( {\eta AP\bar {F}+\bar {\eta }\bar {A}\bar {P}F} \right)+\left( 
%{-\eta BQ\bar {E}+\bar {\eta }\bar {B}\bar {Q}E} \right)} \hfill \\
% {\left( {\eta A\bar {Q}E+\bar {\eta }\bar {A}Q\bar {E}} \right)+\left( 
%{-\eta B\bar {P}F+\bar {\eta }\bar {B}P\bar {F}} \right)} \hfill \\
% {\left( {-\bar {\eta }A\bar {Q}\bar {F}-\eta \bar {A}QF} \right)+\left( 
%{-\bar {\eta }B\bar {P}\bar {E}+\eta \bar {B}PE} \right)} \hfill \\
% {\left( {\bar {\eta }A\bar {Q}\bar {F}-\eta \bar {A}QF} \right)+\left( 
%{\bar {\eta }B\bar {P}\bar {E}+\eta \bar {B}PE} \right)} \hfill \\
% {\left( {\eta A\bar {Q}E-\bar {\eta }\bar {A}Q\bar {E}} \right)+\left( 
%{-\eta B\bar {P}F-\bar {\eta }\bar {B}P\bar {F}} \right)} \hfill \\
% {\left( {\eta AP\bar {F}-\bar {\eta }\bar {A}\bar {P}F} \right)+\left( 
%{-\eta BQ\bar {E}-\bar {\eta }\bar {B}\bar {Q}E} \right)} \hfill \\
% {\left( {-APE+\bar {A}\bar {P}\bar {E}} \right)+\left( {-BQF-\bar {B}\bar 
%{Q}\bar {F}} \right)} \hfill \\
%\end{array} }} \right)
%{\begin{array}{*{20}c}
% {NNN} \hfill \\
% {NNF} \hfill \\
% {NFN} \hfill \\
% {NFF} \hfill \\
% {FNN} \hfill \\
% {FNF} \hfill \\
% {FFN} \hfill \\
% {FFF} \hfill \\
%\end{array} }
\left( {{\begin{array}{*{20}c}
 2Re\left(APE \right)+2Im\left(BQF \right) i \hfill \\
 2Re\left(\eta AP\bar{F} \right)-2Im\left( \eta BQ\bar{E} 
\right)i \hfill \\
 2Re\left(\eta A\bar {Q}E \right)-2Im\left(\eta B\bar {P}F 
\right)i \hfill \\
 -2Re\left(\eta \bar {A}QF \right)+2Im\left( \eta \bar {B}PE
\right)i \hfill \\
 -2Im\left( \eta \bar {A}QF \right)i+2Re\left(\eta \bar {B}PE 
\right) \hfill \\
 2Im\left( \eta A\bar {Q}E \right)i-2Re\left(\eta B\bar {P}F 
\right) \hfill \\
 2Im\left(\eta AP\bar {F} \right)i-2Re\left(\eta BQ\bar {E} 
\right) \hfill \\
 -2Im\left(APE \right)i-2Re\left({BQF} \right) \hfill \\
\end{array} }} \right) %{\begin{array}{*{20}c}
% {NNN} \hfill \\
% {NNF} \hfill \\
% {NFN} \hfill \\
% {NFF} \hfill \\
% {FNN} \hfill \\
% {FNF} \hfill \\
% {FFN} \hfill \\
% {FFF} \hfill \\
%\end{array} }
\]

\subsection{Probability Distribution over the Action Basis}\label{prob}
As per the axioms of quantum mechanics, up to normalization, the referee observing the game state in the 
action basis sees the each basis state according to the following probability distribution.
\[
{\begin{array}{*{20}c}
 pr(NNN)=\left( Re\left[ APE \right] \right)^2+\left( Im\left[ BQF
\right] \right)^2 \hfill \\
 pr(NNF)=\left( Re\left[ {\eta AP\bar 
{F}} \right] \right)^2+\left( Im\left[ \eta BQ\bar {E} \right] 
\right)^2 \hfill \\
 pr(NFN)=\left( Re\left[ \eta A\bar 
{Q}E \right] \right)^2+\left( Im\left[ \eta B\bar {P}F \right] 
\right)^2 \hfill \\
 pr(NFF)=\left( Re\left[ \eta \bar 
{A}QF \right] \right)^2+\left( Im\left[ \eta \bar {B}PE \right]
\right)^2 \hfill \\
 pr(FNN)=\left( {Re\left[ \eta \bar 
{B}PE \right]} \right)^2+\left( Im\left[ \eta \bar {A}QF \right] 
\right)^2 \hfill \\
 pr(FNF)=\left( Re\left[ \eta B\bar 
{P}F \right] \right)^2+\left( Im\left[ \eta A\bar {Q}E \right] 
\right)^2 \hfill \\
 pr(FFN)=\left( Re\left[ \eta BQ\bar 
{E} \right] \right)^2+\left( Im\left[ \eta AP\bar {F} \right] 
\right)^2 \hfill \\
 pr(FFF)=\left( Re\left[ {BQF} \right] \right)^2+\left( Im\left[ {APE} 
\right] \right)^2 \hfill \\
\end{array} }
\]
Now let
$$
A=a_0 +a_1 i,\;\; B=b_0 +b_1 i
$$
$$
P=p_0 +q_1 i,\;\; Q=q_0 +q_1i
$$
$$
E=e_0 +e_1 i,\;\; F=f_0 +f_1 i.
$$ 
Then the above probability distribution over the action basis can be expressed as
\begin{eqnarray*}
pr(NNN) &=& \left( b_0 q_0 f_1 +b_0 q_1 f_0 +b_1 q_0 f_0 -b_1 q_1 f_1  \right)^2 \\
&+& \left( a_0 p_0 e_0 -a_0 p_1 e_1 -a_1 p_0 e_1 -a_1p_1 e_0  \right)^2
\end{eqnarray*}
\begin{eqnarray*}
pr(NNF) &=& [\frac{1}{2}(-b_0 q_0 e_1 +b_0 q_1 e_0 +b_1 q_0 e_0 +b_1 q_1 e_1)\\
&+& \frac{\sqrt 3}{2}(b_0 q_0 e_0 +b_0 q_1 e_1 + b_1 q_0 e_1 -b_1 q_1 e_0) ]^2 \\
&+& [\frac{1}{2}(a_0 p_0 f_0 +a_0 p_1 f_1 +a_1 p_0 f_1 -a_1 p_1 f_1)\\
&+& \frac{\sqrt 3}{2}(a_0 p_0 f_1 -a_0 p_1 f_0 -a_1 p_0 f_0 -a_1 p_1 f_1) ]^2
\end{eqnarray*}
\begin{eqnarray*}
pr(NFN) &=& [ \frac{1}{2}\left( a_0 q_0 e_0 +a_0 q_1 e_1 -a_1 q_0 e_1 +a_1 q_1 e_0  \right)\\
&+& \frac{\sqrt 3 }{2}\left( -a_0 q_0 e_1 +a_0 q_1 e_0 -a_1 q_0 e_0 -a_1 q_1 e_1  \right) ]^2 \\ 
&+& [ \frac{1}{2}\left( b_0 p_0 f_1 -b_0 p_1 f_0 +b_1 p_0 f_0 +b_1 p_1 f_1  \right)\\
&+& \frac{\sqrt 3 }{2}\left( b_0 p_0 f_0 +b_0 p_1 f_1 -b_1 p_0 f_1 +b_1 p_1 f_0  \right) ]^2 
\end{eqnarray*}
\begin{eqnarray*}
pr(NFF) &=& [ \frac{1}{2}\left( a_0 q_0 f_0 -a_0 q_1 f_1 +a_1 q_0 f_1 +a_1 q_1 f_0  \right)\\
&+& \frac{\sqrt 3 }{2}\left( -a_0 q_0 f_1 -a_0 q_1 f_0+a_1 q_0 f_0 -a_1 q_1 f_1  \right)]^2 \\
&+& [ \frac{1}{2}\left( b_0 p_0 e_1 +b_0 p_1 e_0 -b_1 p_0 e_0 +b_1 p_1 e_1 \right)\\
&+& \frac{\sqrt 3}{2}\left( b_0 p_0 e_0 -b_0 p_1 e_1 +b_1 p_0 f_1 +b_1 p_1 e_0 \right) ]^2
\end{eqnarray*}
\begin{eqnarray*}
pr(FNN) &=& [ \frac{1}{2}\left( a_0 q_0 f_1 +a_0 q_1 f_0 -a_1 q_0 f_0 +a_1 q_1 f_1  \right)\\
&+& \frac{\sqrt 3}{2}\left( a_0 q_0 f_0 -a_0 q_1 f_1 +a_1 q_0 f_1 +a_1 q_1 f_0  \right)]^2 \\ 
&+& [ \frac{1}{2}\left( b_0 p_0 e_0 -b_0 p_1 e_1 +b_1 p_0 f_1 +b_1 p_1 e_0  \right)\\
&+& \frac{\sqrt 3 }{2}\left( -b_0 p_0 e_1 -b_0 p_1 e_0 +b_1 p_0 e_0 -b_1 p_1 e_1  \right) ]^2 
\end{eqnarray*}
\begin{eqnarray*}
pr(FNN) &=& [ \frac{1}{2}\left( a_0 q_0 f_1 +a_0 q_1 f_0 -a_1 q_0 f_0 +a_1 q_1 f_1  \right)\\
&+& \frac{\sqrt 3 }{2}\left( a_0 q_0 f_0 -a_0 q_1 f_1 +a_1 q_0 f_1 +a_1 q_1 f_0  \right) ]^2 \\ 
&+& [ \frac{1}{2}\left( b_0 p_0 e_0 -b_0 p_1 e_1 +b_1 p_0 f_1 +b_1 p_1 e_0  \right)\\
&+& \frac{\sqrt 3}{2}\left( -b_0 p_0 e_1 -b_0 p_1 e_0 +b_1 p_0 e_0 -b_1 p_1 e_1  \right) ]^2 
\end{eqnarray*}
\begin{eqnarray*}
pr(FNF)&=& [ \frac{1}{2}\left( a_0 q_0 e_1 -a_0 q_1 e_0 +a_1 q_0 e_0 +a_1 q_1 e_1 \right)\\
&+& \frac{\sqrt 3 }{2}\left( a_0 q_0 e_0 +a_0 q_1 e_1 -a_1 q_0 e_1 +a_1 q_1 e_0 \right)]^2 \\ 
&+& [ \frac{1}{2}\left( b_0 p_0 f_0 +b_0 p_1 f_1 -b_1 p_0 f_1 +b_1 p_1 f_0  \right)\\
&+& \frac{\sqrt 3 }{2}\left( -b_0 p_0 f_1 +b_0 p_1 f_0 -b_1 p_0 f_0 -b_1 p_1 f_1 \right)]^2 
\end{eqnarray*}
\begin{eqnarray*}
pr(FFN) &=& [ \frac{1}{2}\left( b_0 q_0 e_0 +b_0 q_1 e_1 +b_1 q_0 e_1 -b_1 q_1 e_0  \right)\\
&+& \frac{\sqrt 3 }{2}\left( b_0 q_0 e_1 -b_0 q_1 e_0 -b_1 q_0 e_0 -b_1 q_1 e_1  \right)]^2 \\ 
&+& [ \frac{1}{2}\left( -a_0 p_0 f_1 +a_0 p_1 f_0 +a_1 p_0 f_0 +a_1 p_1 f_1  \right)\\
&+& \frac{\sqrt 3 }{2}\left( a_0 p_0 f_0 +a_0 p_1 f_1 +a_1 p_0 f_1 -a_1 p_1 f_0 \right)]^2 
\end{eqnarray*}
\begin{eqnarray*}
pr(FFF)&=& \left( b_0 q_0 f_0 -b_0 q_1 f_1 -b_1 q_0 f_1 -b_1 q_1 f_0 \right)^2\\
&+& \left( a_0 p_0 e_1 +a_0 p_1 e_0 +a_1 p_0 e_0 -a_1p_1 e_1  \right)^2
\end{eqnarray*}

\subsection{Proof of Theorem \ref{theorem}}
All that remains now to prove theorem \ref{theorem} is to reconcile the expressions of the probability distribution in section \ref{prob} with the octonionic formulae of theorem \ref{theorem}.

Recall that these octonionic formulae arose from the identification of the players' classical strategy sets with quaternionic subspace of the octonions. In turn, we identified an arbitrary strategy of players 1, 2, and 3 respectively with the following unit octionions.
\begin{align*}
 s_{00} &\equiv A+B\bar {\eta }i_4 =a_0 +a_1 i_1 +\left( {b_0 +b_1 i_1 } 
\right)\left( {\frac{1}{2}-\frac{\sqrt 3 }{2}i_1 } \right)i_4 \\ 
&=a_0 +a_1 i_1 +\left( {\frac{\sqrt 3 }{2}b_0 -\frac{1}{2}b_1 } 
\right)i_2 +\left( {\frac{1}{2}b_0 +\frac{\sqrt 3 }{2}b_1 } \right)i_4 
\end{align*}
\begin{align*}
 t_{00} &\equiv P+Q\bar {\eta }i_6 =p_0 +p_1 i_1 +\left( {q_0 +q_1 i_1 } 
\right)\left( {\frac{1}{2}-\frac{\sqrt 3 }{2}i_1 } \right)i_6 \\ 
&=p_0 +p_1 i_1 +\left( {\frac{\sqrt 3 }{2}q_0 -\frac{1}{2}q_1 } 
\right)i_5 +\left( {\frac{1}{2}q_0 +\frac{\sqrt 3 }{2}q_1 } \right)i_6 
\end{align*}
\begin{align*}
 u_{00} &\equiv E+F\bar {\eta }i_7 =e_0 +e_1 i_1 +\left( {f_0 +f_1 i_1 } 
\right)\left( {\frac{1}{2}-\frac{\sqrt 3 }{2}i_1 } \right)i_7 \\ 
&=e_0 +e_1 i_1 +\left( {\frac{\sqrt 3 }{2}f_0 -\frac{1}{2}f_1 } 
\right)i_3 +\left( {\frac{1}{2}f_0 +\frac{\sqrt 3 }{2}f_1 } \right)i_7
\end{align*}
The proof of theorem \ref{theorem} will require the use of the following octonions as well.
\[
 s_{10} =-a_0 +a_1 i_1 +\left( {\frac{\sqrt 3 }{2}b_0 -\frac{1}{2}b_1 } 
\right)i_2 +\left( {\frac{1}{2}b_0 +\frac{\sqrt 3 }{2}b_1 } \right)i_4
\]
\[
 s_{01} =a_0 -a_1 i_1 +\left( {\frac{\sqrt 3 }{2}b_0 -\frac{1}{2}b_1 } 
\right)i_2 +\left( {\frac{1}{2}b_0 +\frac{\sqrt 3 }{2}b_1 } \right)i_4 
\]
\[
 t_{10} =-p_0 +p_1 i_1 +\left( {\frac{\sqrt 3 }{2}q_0 -\frac{1}{2}q_1 } 
\right)i_5 +\left( {\frac{1}{2}q_0 +\frac{\sqrt 3 }{2}q_1 } \right)i_6 
\]
\[
 u_{01} =e_0 -e_1 i_1 +\left( {\frac{\sqrt 3 }{2}f_0 -\frac{1}{2}f_1 } 
\right)i_3 +\left( {\frac{1}{2}f_0 +\frac{\sqrt 3 }{2}f_1 } \right)i_7 
\]
For any octonion $o$, denote by $\pi _k (o)$ the projection of the octonion 
$o$ onto the subspace of $\mathbb{O}$ spanned by the vector basis element $i_k $. %Then our goal 
%is to show that
%\[
%\begin{array}{l}
% pr(NNN)=\left[ {\pi _0 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} 
%+\left( {s_{01} t_{10} } \right)u_{01} }{2}} \right)} \right]^2+\left[ {\pi 
%_0 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} -\left( {s_{01} 
%t_{10} } \right)u_{01} }{2}} \right)} \right]^2 \\ 
% pr(FFF)=\left[ {\pi _1 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} 
%+\left( {s_{01} t_{10} } \right)u_{01} }{2}} \right)} \right]^2+\left[ {\pi 
%_1 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} -\left( {s_{01} 
%t_{10} } \right)u_{01} }{2}} \right)} \right]^2 \\ 
% pr(FFN)=\left[ {\pi _3 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} 
%+\left( {s_{01} t_{10} } \right)u_{01} }{2}} \right)} \right]^2+\left[ {\pi 
%_3 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} -\left( {s_{01} 
%t_{10} } \right)u_{01} }{2}} \right)} \right]^2 \\ 
% pr(NNF)=\left[ {\pi _7 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} 
%+\left( {s_{01} t_{10} } \right)u_{01} }{2}} \right)} \right]^2+\left[ {\pi 
%_7 \left( {\frac{\left( {s_{10} t_{10} } \right)u_{01} -\left( {s_{01} 
%t_{10} } \right)u_{01} }{2}} \right)} \right]^2 \\ 
% pr(NFF)=\left[ {\pi _2 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} 
%+\left( {s_{01} t_{00} } \right)u_{00} }{2}} \right)} \right]^2+\left[ {\pi 
%_2 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} -\left( {s_{01} 
%t_{00} } \right)u_{00} }{2}} \right)} \right]^2 \\ 
% pr(FNN)=\left[ {\pi _4 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} 
%+\left( {s_{01} t_{00} } \right)u_{00} }{2}} \right)} \right]^2+\left[ {\pi 
%_4 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} -\left( {s_{01} 
%t_{00} } \right)u_{00} }{2}} \right)} \right]^2 \\ 
% pr(FNF)=\left[ {\pi _5 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} 
%+\left( {s_{01} t_{00} } \right)u_{00} }{2}} \right)} \right]^2+\left[ {\pi 
%_5 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} -\left( {s_{01} 
%t_{00} } \right)u_{00} }{2}} \right)} \right]^2 \\ 
% pr(NFN)=\left[ {\pi _6 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} 
%+\left( {s_{01} t_{00} } \right)u_{00} }{2}} \right)} \right]^2+\left[ {\pi 
%_6 \left( {\frac{\left( {s_{10} t_{00} } \right)u_{00} -\left( {s_{01} 
%t_{00} } \right)u_{00} }{2}} \right)} \right]^2 \\ 
% \end{array}
%\]
Now note that:
 %pr(NNN)=\left( {b_0 q_0 f_1 +b_0 q_1 f_0 +b_1 q_0 f_0 -b_1 q_1 f_1 } 
%\right)^2+\left( {a_0 p_0 e_0 -a_0 p_1 e_1 -a_1 p_0 e_1 -a{ }_1p_1 e_0 } 
%\right)^2 \\
\[
 \pi _0 \left[ \frac{(s_{10} t_{10} )u_{01} +(s_{01} t_{10})u_{01} }{2} \right]=-b_0 q_0 f_1 -b_0 q_1 f_0 -b_1 q_0 f_0 +b_1 q_1 f_1
\]
\[
 \pi _0 \left[ {\frac{(s_{10} t_{10} )u_{01} -(s_{01} t_{10} )u_{01} }{2}} 
\right]=a_0 p_0 e_0 -a_0 p_1 e_1 -a_1 p_0 e_1 -a{ }_1p_1 e_0 
\]
and that
\begin{eqnarray*}
 pr(NNN) &=& \left( \pi _0 \left[ \frac{(s_{10} t_{10} )u_{01} +(s_{01} t_{10} 
)u_{01} }{2} \right] \right)^2\\
&+& \left( \pi _0 \left[ \frac{(s_{10} t_{10} 
)u_{01} -(s_{01} t_{10} )u_{01} }{2} \right] \right)^2
\end{eqnarray*}
Similarly, we make the following reconciliations:
\begin{enumerate}
\item  Probability of observing the state $FFF$:
\[
% pr(FFF)=\left( {b_0 q_0 f_0 -b_0 q_1 f_1 -b_1 q_0 f_1 -b_1 q_1 f_0 } 
%\right)^2+\left( {a_0 p_0 e_1 +a_0 p_1 e_0 +a_1 p_0 e_0 -a{ }_1p_1 e_1 } 
%\right)^2 \\ 
 \pi _1 \left[ {\frac{(s_{10} t_{10} )u_{01} +(s_{01} t_{10} )u_{01} }{2}} 
\right]=-b_0 q_0 f_0 +b_0 q_1 f_1 +b_1 q_0 f_1 +b_1 q_1 f_0 
\]
\[
 \pi _1 \left[ {\frac{(s_{10} t_{10} )u_{01} -(s_{01} t_{10} )u_{01} }{2}} 
\right]=-a_0 p_0 e_1 -a_0 p_1 e_0 -a_1 p_0 e_0 +a{ }_1p_1 e_1
\]
and
\begin{eqnarray*}
 pr(FFF) &=& \left( \pi _1 \left[ \frac{(s_{10} t_{10} )u_{01} +(s_{01} t_{10} 
)u_{01} }{2} \right] \right)^2\\
&+& \left( \pi _1 \left[ \frac{(s_{10} t_{10} 
)u_{01} -(s_{01} t_{10} )u_{01} }{2} \right] \right)^2 \\ 
\end{eqnarray*}
\item Probability of observing the state $NNF$:
\begin{align*}
%
% pr(NNF)=\left[ {\frac{1}{2}\left( {-b_0 q_0 e_1 +b_0 q_1 e_0 +b_1 q_0 e_0 
%+b_1 q_1 e_1 } \right)+\frac{\sqrt 3 }{2}\left( {b_0 q_0 e_0 +b_0 q_1 e_1 
%+b_1 q_0 e_1 -b_1 q_1 e_0 } \right)} \right]^2 \\ 
% \;\;\;\;\;\;\;\;\;\;\;\;+\left[ {\frac{1}{2}\left( {a_0 p_0 f_0 +a_0 p_1 
%f_1 +a_1 p_0 f_1 -a_1 p_1 f_0 } \right)+\frac{\sqrt 3 }{2}\left( {a_0 p_0 
%f_1 -a_0 p_1 f_0 -a_1 p_0 f_0 -a_1 p_1 f_1 } \right)} \right]^2 \\ 
 \pi _7 \left[ {\frac{(s_{10} t_{10} )u_{01} +(s_{01} t_{10} )u_{01} }{2}} 
\right]&=\frac{1}{2}\left( {-b_0 q_0 e_1 +b_0 q_1 e_0 +b_1 q_0 e_0 +b_1 q_1 
e_1 } \right)\\
&+\frac{\sqrt 3 }{2}\left( {b_0 q_0 e_0 +b_0 q_1 e_1 +b_1 q_0 
e_1 -b_1 q_1 e_0 } \right)
\end{align*}
\begin{align*}
 \pi _7 \left[ {\frac{(s_{10} t_{10} )u_{01} -(s_{01} t_{10} )u_{01} }{2}} 
\right]&=\frac{1}{2}\left( {a_0 p_0 f_0 +a_0 p_1 f_1 +a_1 p_0 f_1 -a_1 p_1 
f_0 } \right)\\
&+\frac{\sqrt 3 }{2}\left( {a_0 p_0 f_1 -a_0 p_1 f_0 -a_1 p_0 
f_0 -a_1 p_1 f_1 } \right)
\end{align*}
and
\begin{eqnarray*}
pr(NNF)&=& \left( \pi _7 \left[ \frac{(s_{10} t_{10} )u_{01} +(s_{01} t_{10} 
)u_{01} }{2} \right] \right)^2\\
&+& \left( \pi _7 \left[ \frac{(s_{10} t_{10} 
)u_{01} -(s_{01} t_{10} )u_{01} }{2} \right] \right)^2
\end{eqnarray*}
\item Probability of observing the state $FFN$:
\begin{align*}
 %pr(FFN)=\left[ {\frac{1}{2}\left( {b_0 q_0 e_0 +b_0 q_1 e_1 +b_1 q_0 e_1 
%-b_1 q_1 e_0 } \right)+\frac{\sqrt 3 }{2}\left( {b_0 q_0 e_1 -b_0 q_1 e_0 
%-b_1 q_0 e_0 -b_1 q_1 e_1 } \right)} \right]^2 \\ 
% \;\;\;\;\;\;\;\;\;\;\;\;+\left[ {\frac{1}{2}\left( {-a_0 p_0 f_1 +a_0 p_1 
%f_0 +a_1 p_0 f_0 +a_1 p_1 f_1 } \right)+\frac{\sqrt 3 }{2}\left( {a_0 p_0 
%f_0 +a_0 p_1 f_1 +a_1 p_0 f_1 -a_1 p_1 f_0 } \right)} \right]^2 \\ 
\pi _3 \left[ {\frac{(s_{10} t_{10} )u_{01} +(s_{01} t_{10} )u_{01} }{2}} 
\right]&=\frac{1}{2}\left( {-b_0 q_0 e_0 -b_0 q_1 e_1 -b_1 q_0 e_1 +b_1 q_1 
e_0 } \right)\\
&+\frac{\sqrt 3 }{2}\left( {-b_0 q_0 e_1 +b_0 q_1 e_0 +b_1 q_0 
e_0 +b_1 q_1 e_1 )} \right)
\end{align*}
\begin{align*}
 \pi _3 \left[ {\frac{(s_{10} t_{10} )u_{01} -(s_{01} t_{10} )u_{01} }{2}} 
\right]&=\frac{1}{2}\left( {-a_0 p_0 f_1 +a_0 p_1 f_0 +a_1 p_0 f_0 +a_1 p_1 
f_1 } \right)\\
&+\frac{\sqrt 3 }{2}\left( {a_0 p_0 f_0 +a_0 p_1 f_1 +a_1 p_0 
f_1 -a_1 p_1 f_0 } \right) 
\end{align*}
and
\begin{eqnarray*}
pr(FFN) &=& \left( \pi _3 \left[ \frac{(s_{10} t_{10} )u_{01} +(s_{01} t_{10} 
)u_{01} }{2} \right] \right)^2\\
&+& \left( \pi _3 \left[ \frac{(s_{10} t_{10} 
)u_{01} -(s_{01} t_{10} )u_{01} }{2} \right] \right)^2 
\end{eqnarray*}
\item Probability of observing the state $NFF$:
\begin{align*}
%
% pr(NFF)=\left[ {\frac{1}{2}\left( {a_0 q_0 f_0 -a_0 q_1 f_1 +a_1 q_0 f_1 
%+a_1 q_1 f_0 } \right)+\frac{\sqrt 3 }{2}\left( {-a_0 q_0 f_1 -a_0 q_1 f_0 
%+a_1 q_0 f_0 -a_1 q_1 f_1 } \right)} \right]^2 \\ 
% \;\;\;\;\;\;\;\;\;\;\;\;+\left[ {\frac{1}{2}\left( {b_0 p_0 e_1 +b_0 p_1 
%e_0 -b_1 p_0 e_0 +b_1 p_1 e_1 } \right)+\frac{\sqrt 3 }{2}\left( {b_0 p_0 
%e_0 -b_0 p_1 e_1 +b_1 p_0 f_1 +b_1 p_1 e_0 } \right)} \right]^2 \\ 
 \pi _2 \left[ {\frac{(s_{10} t_{00} )u_{00} +(s_{01} t_{00} )u_{00} }{2}} 
\right]&=\frac{1}{2}\left( {a_0 q_0 f_0 -a_0 q_1 f_1 +a_1 q_0 f_1 +a_1 q_1 
f_0 } \right)\\
&+\frac{\sqrt 3 }{2}\left( {-a_0 q_0 f_1 -a_0 q_1 f_0 +a_1 q_0 
f_0 -a_1 q_1 f_1 } \right)
\end{align*}
\begin{align*}
 \pi _2 \left[ {\frac{(s_{10} t_{00} )u_{00} -(s_{01} t_{00} )u_{00} }{2}} 
\right]&=\frac{1}{2}\left( {b_0 p_0 e_1 +b_0 p_1 e_0 -b_1 p_0 e_0 +b_1 p_1 
e_1 } \right)\\
&+\frac{\sqrt 3 }{2}\left( {b_0 p_0 e_0 -b_0 p_1 e_1 +b_1 p_0 
f_1 +b_1 p_1 e_0 } \right)
\end{align*}
and
\begin{eqnarray*}
pr(NFF) &=& \left( \pi _2 \left[ \frac{(s_{10} t_{00} )u_{00} +(s_{01} t_{00} 
)u_{00} }{2} \right] \right)^2\\
&+& \left( \pi _2 \left[ \frac{(s_{10} t_{00} 
)u_{00} -(s_{01} t_{00} )u_{00} }{2} \right] \right)^2 
\end{eqnarray*}
\item Probability of observing the state $FNN$:
\begin{align*}
% pr(FNN)=\left[ {\frac{1}{2}\left( {a_0 q_0 f_1 +a_0 q_1 f_0 -a_1 q_0 f_0 
%+a_1 q_1 f_1 } \right)+\frac{\sqrt 3 }{2}\left( {a_0 q_0 f_0 -a_0 q_1 f_1 
%+a_1 q_0 f_1 +a_1 q_1 f_0 } \right)} \right]^2 \\ 
% \;\;\;\;\;\;\;\;\;\;\;\;+\left[ {\frac{1}{2}\left( {b_0 p_0 e_0 -b_0 p_1 
%e_1 +b_1 p_0 f_1 +b_1 p_1 e_0 } \right)+\frac{\sqrt 3 }{2}\left( {-b_0 p_0 
%e_1 -b_0 p_1 e_0 +b_1 p_0 e_0 -b_1 p_1 e_1 } \right)} \right]^2 \\ 
 \pi _4 \left[ {\frac{(s_{10} t_{00} )u_{00} +(s_{01} t_{00} )u_{00} }{2}} 
\right]&=\frac{1}{2}\left( {b_0 p_0 e_0 -b_0 p_1 e_1 +b_1 p_0 f_1 +b_1 p_1 
e_0 } \right)\\
&+\frac{\sqrt 3 }{2}\left( {-b_0 p_0 e_1 -b_0 p_1 e_0 +b_1 p_0 
e_0 -b_1 p_1 e_1 } \right)
\end{align*}
\begin{align*}
 \pi _4 \left[ {\frac{(s_{10} t_{00} )u_{00} -(s_{01} t_{00} )u_{00} }{2}} 
\right]&=\frac{1}{2}\left( {-a_0 q_0 f_1 -a_0 q_1 f_0 +a_1 q_0 f_0 -a_1 q_1 
f_1 } \right)\\
&+\frac{\sqrt 3 }{2}\left( {-a_0 q_0 f_0 +a_0 q_1 f_1 -a_1 q_0 
f_1 -a_1 q_1 f_0 } \right)
\end{align*}
and
\begin{eqnarray*}
 pr(FNN)&=& \left( \pi _4 \left[ \frac{(s_{10} t_{00} )u_{00} +(s_{01} t_{00} 
)u_{00} }{2} \right] \right)^2\\
&+& \left( \pi _4 \left[ \frac{(s_{10} t_{00} 
)u_{00} -(s_{01} t_{00} )u_{00} }{2} \right] \right)^2
\end{eqnarray*}
\item Probability of observing the state $FNF$:
\begin{align*}
% pr(FNF)=\left[ {\frac{1}{2}\left( {a_0 q_0 e_1 -a_0 q_1 e_0 +a_1 q_0 e_0 
%+a_1 q_1 e_1 } \right)+\frac{\sqrt 3 }{2}\left( {a_0 q_0 e_0 +a_0 q_1 e_1 
%-a_1 q_0 e_1 +a_1 q_1 e_0 } \right)} \right]^2 \\ 
% \;\;\;\;\;\;\;\;\;\;\;\;+\left[ {\frac{1}{2}\left( {b_0 p_0 f_0 +b_0 p_1 
%f_1 -b_1 p_0 f_1 +b_1 p_1 f_0 } \right)+\frac{\sqrt 3 }{2}\left( {-b_0 p_0 
%f_1 +b_0 p_1 f_0 -b_1 p_0 f_0 -b_1 p_1 f_1 } \right)} \right]^2 \\ 
 \pi _5 \left[ {\frac{(s_{10} t_{00} )u_{00} +(s_{01} t_{00} )u_{00} }{2}} 
\right]&=\frac{1}{2}\left( {b_0 p_0 f_0 +b_0 p_1 f_1 -b_1 p_0 f_1 +b_1 p_1 
f_0 } \right)\\
&+\frac{\sqrt 3 }{2}\left( {-b_0 p_0 f_1 +b_0 p_1 f_0 -b_1 p_0 
f_0 -b_1 p_1 f_1 } \right)
\end{align*}
\begin{align*} 
 \pi _5 \left[ {\frac{(s_{10} t_{00} )u_{00} -(s_{01} t_{00} )u_{00} }{2}} 
\right]&=\frac{1}{2}\left( {-a_0 q_0 e_1 +a_0 q_1 e_0 -a_1 q_0 e_0 -a_1 q_1 
e_1 } \right)\\
&+\frac{\sqrt 3 }{2}\left( {-a_0 q_0 e_0 -a_0 q_1 e_1 +a_1 q_0 
e_1 -a_1 q_1 e_0 } \right)
\end{align*}
and
\begin{eqnarray*}
 pr(FNF) &=& \left( \pi _5 \left[ \frac{(s_{10} t_{00} )u_{00} +(s_{01} t_{00} 
)u_{00} }{2} \right] \right)^2\\
&+& \left( \pi _5 \left[ \frac{(s_{10} t_{00} 
)u_{00} -(s_{01} t_{00} )u_{00} }{2} \right] \right)^2
\end{eqnarray*}
\item Probability of observing the state $NFN$:
\begin{align*}
% pr(NFN)=\left[ {\frac{1}{2}\left( {a_0 q_0 e_0 +a_0 q_1 e_1 -a_1 q_0 e_1 
%+a_1 q_1 e_0 } \right)+\frac{\sqrt 3 }{2}\left( {-a_0 q_0 e_1 +a_0 q_1 e_0 
%-a_1 q_0 e_0 -a_1 q_1 e_1 } \right)} \right]^2 \\ 
% \;\;\;\;\;\;\;\;\;\;\;\;+\left[ {\frac{1}{2}\left( {b_0 p_0 f_1 -b_0 p_1 
%f_0 +b_1 p_0 f_0 +b_1 p_1 f_1 } \right)+\frac{\sqrt 3 }{2}\left( {b_0 p_0 
%f_0 +b_0 p_1 f_1 -b_1 p_0 f_1 +b_1 p_1 f_0 } \right)} \right]^2 \\ 
 \pi _6 \left[ {\frac{(s_{10} t_{00} )u_{00} +(s_{01} t_{00} )u_{00} }{2}} 
\right]&=\frac{1}{2}\left( {b_0 p_0 f_0 +b_0 p_1 f_1 -b_1 p_0 f_1 +b_1 p_1 
f_0 } \right)\\
&+\frac{\sqrt 3 }{2}\left( {-b_0 p_0 f_1 +b_0 p_1 f_0 -b_1 p_0 
f_0 -b_1 p_1 f_1 } \right)
\end{align*} 
\begin{align*}
 \pi _6 \left[ {\frac{(s_{10} t_{00} )u_{00} -(s_{01} t_{00} )u_{00} }{2}} 
\right]&=\frac{1}{2}\left( {-a_0 q_0 e_1 +a_0 q_1 e_0 -a_1 q_0 e_0 -a_1 q_1 
e_1 } \right)\\
&+\frac{\sqrt 3 }{2}\left( {-a_0 q_0 e_0 -a_0 q_1 e_1 +a_1 q_0 
e_1 -a_1 q_1 e_0 } \right) 
\end{align*}
and
\begin{eqnarray*}
pr(NFN) &=& \left( \pi _6 \left[ \frac{(s_{10} t_{00} )u_{00} +(s_{01} t_{00} 
)u_{00} }{2} \right] \right)^2\\
&+& \left( \pi _6 \left[ \frac{(s_{10} t_{00} 
)u_{00} -(s_{01} t_{00} )u_{00} }{2} \right] \right)^2 
\end{eqnarray*}
\end{enumerate}

\section{A Special Discrete Distribution}

Consider a three player, two strategy game with the following payoff matrix

\begin{longtable}[htbp]
{|p{30pt}|p{30pt}|p{30pt}|p{30pt}|p{30pt}|p{30pt}|p{30pt}|p{30pt}|p{30pt}|}
\hline
\endhead
\hline
\endfoot
III \par II \par I \par & 
Z$_{0}$ \par Y$_{0}$ \par X$_{0}$& 
Z$_{7}$ \par Y$_{7}$ \par X$_{7}$& 
Z$_{6}$ \par Y$_{6}$ \par X$_{6}$& 
Z$_{2}$ \par Y$_{2}$ \par X$_{2}$& 
Z$_{4}$ \par Y$_{4}$ \par X$_{4}$& 
Z$_{5}$ \par Y$_{5}$ \par X$_{5}$ & 
Z$_{3}$ \par Y$_{3}$ \par X$_{3}$& 
Z$_{1}$ \par Y$_{1}$ \par X$_{1}$  \\
\hline
Players& 
NNN \par 1& 
NNF \par $i_7 $& 
NFN \par $i_6 $& 
NFF \par $i_2 $& 
FNN \par $i_4 $& 
FNF \par $i_5 $& 
FFN \par $i_3 $& 
FFF \par $i_1 $
\label{tab2}
\end{longtable}
\noindent where the X$_{t}$'s, Y$_{t}$'s, and Z$_{t}$'s are all real numbers.

\begin{definition}{\rm
Define a \emph{discrete distribution} as a mixed strategy 
that is supported on a finite number of points. }
\end{definition}

One such discrete distribution is the distribution where each player 
plays his pure strategy corresponding to a single octonionic basis element 
with probability $\frac{1}{4}$. In particular, for player 1, 
this is the mixed quantum strategy 
$$
\sigma =\frac{1}{4}+\frac{1}{4}i_1 
+\frac{1}{4}i_2 +\frac{1}{4}i_4,
$$ 
for player 2
$$\tau =\frac{1}{4}+\frac{1}{4}i_1 +\frac{1}{4}i_5 +\frac{1}{4}i_6,
$$
and for player 3
$$
\upsilon =\frac{1}{4}+\frac{1}{4}i_1 +\frac{1}{4}i_3 
+\frac{1}{4}i_7. 
$$
Suppose that players 1, 2, and 3 use the mixed quantum strategies $\sigma$, $\tau$ and $\upsilon$, respectively. Then the expected payoff to player 
$k$ is given by
\begin{align*}
&\sum _k (\sigma ,\tau ,\upsilon )=\\
&\frac{1}{64}[P_k (1,1,1)+P_k (1,1,i_1)+P_k (1,1,i_3 )+P_k (1,1,i_7 )+P_k(1,i_1 ,1)\\
&+P_k (1,i_1 ,i_1 )+P_k (1,i_1 ,i_3)+P_k (1,i_1 ,i_7 )+P_k (1,i_5 ,1)+P_k (1,i_5 ,i_1 )\\
&+P_k (1,i_5,i_3 )+P_k (1,i_5 ,i_7 )+P_k (1,i_6 ,1)+P_k (1,i_6 ,i_1 )+P_k (1,i_6 ,i_3)\\
&+P_k (1,i_6 ,i_7 )+P_k (i_1 ,1,1)+P_k (i_1 ,1,i_1 )+P_k (i_1,1,i_3 )+P_k (i_1 ,1,i_7 )\\
&+P_k (i_1 ,i_1 ,1)+P_k (i_1 ,i_1 ,i_1 )+P_k (i_1,i_1 ,i_3 )+P_k (i_1 ,i_1 ,i_7 )+P_k (i_1 ,i_5 ,1)\\
&+P_k (i_1 ,i_5 ,i_1 )+P_k(i_1 ,i_5 ,i_3 )+P_k (i_1 ,i_5 ,i_7 )+P_k (i_1 ,i_6 ,1)+P_k (i_1 ,i_6 ,i_1)\\
&+P_k (i_1 ,i_6 ,i_3 )+P_k (i_1 ,i_6 ,i_7 )+P_k (i_2 ,1,1)+P_k (i_2 ,1,i_1 )+P_k (i_2 ,1,i_3)\\
&+P_k (i_2 ,1,i_7 )+P_k (i_2 ,i_1 ,1)+P_k (i_2 ,i_1 ,i_1 )+P_k (i_2 ,i_1,i_3 )+P_k (i_2 ,i_1 ,i_7 )\\
&+P_k (i_2 ,i_5 ,1)+P_k (i_2 ,i_5 ,i_1 )+P_k (i_2,i_5 ,i_3 )+P_k (i_2 ,i_5 ,i_7 )+P_k (i_2 ,i_6 ,1)\\
&+P_k (i_2 ,i_6 ,i_1 )+P_k(i_2 ,i_6 ,i_3 )+P_k (i_2 ,i_6 ,i_7 ) +P_k (i_4 ,1,1)+P_k (i_4 ,1,i_1 )\\
&+P_k (i_4 ,1,i_3)+P_k (i_4 ,1,i_7 )+P_k (i_4 ,i_1 ,1)+P_k (i_4 ,i_1 ,i_1 )+P_k (i_4 ,i_1 ,i_3 )\\
&+P_k (i_4 ,i_1 ,i_7 )+P_k (i_4 ,i_5 ,1)+P_k (i_4 ,i_5 ,i_1 )+P_k (i_4,i_5 ,i_3 )+P_k (i_4 ,i_5 ,i_7 )\\
&+P_k (i_4 ,i_6 ,1)+P_k (i_4 ,i_6 ,i_1 )+P_k(i_4 ,i_6 ,i_3 )+P_k (i_4 ,i_6 ,i_7 )]
 \end{align*}
Simplifying the above expression will require the use of the following 
corollary to Theorem \ref{theorem}.

\begin{corollary}\label{coro}{\rm
If $s$ is any element of the set $\{1,i_1,i_2,i_4 \}$, $t$ any element 
of the set $\{1, i_1, i_5, i_6 \}$, and $u$ any element of the set $\{1, i_1, i_3, i_7\}$, then the conclusion of Theorem \ref{theorem} reduces to}
\[
\begin{array}{l}
 pr(NNN)=\left[ {\pi _0 \left( {(st)u} \right)} 
\right]^2\;\;\;\;\;pr(FFF)=\left[ {\pi _1 \left( {(st)u} \right)} \right]^2 
\\ 
 pr(FFN)=\left[ {\pi _3 \left( {(st)u} \right)} 
\right]^2\;\;\;\;\;pr(NNF)=\left[ {\pi _7 \left( {(st)u} \right)} \right]^2 
\\ 
 pr(NFF)=\left[ {\pi _2 \left( {(st)u} \right)} 
\right]^2\;\;\;\;\;pr(FNN)=\left[ {\pi _4 \left( {(st)u} \right)} \right]^2 
\\ 
 pr(FNF)=\left[ {\pi _5 \left( {(st)u} \right)} 
\right]^2\;\;\;\;\;pr(NFN)=\left[ {\pi _6 \left( {(st)u} \right)} \right]^2 
\\ 
 \end{array}
\]
\end{corollary}

\begin{proof}
We need to check 64 cases. We will go over one and leave the remaining 63 as 
an exercise for the reader.
\end{proof}

That is, if players employ single octonionic basis elements as strategies, 
then the payoff to player $k$ is given by 
$$P_k (s,t,u)=\sum\limits_{l=0}^7 
{\left[ {\pi _l \left( {(st)u} \right)} \right]} ^2W_t,
$$
where $W$ is $X$ for 
player 1, $Y$ for player 2, and $Z$ for player 3.

If $s=i_4$, $t=i_6$, and $u=i_7 $, then $s_{10}=s_{01}=s$, $t_{10} 
=t_{00}=t$, and $u_{01}=u_{00}=u$. Thus 
$$
\frac{\left( {s_{10} 
t_{10} } \right)u_{01} +\left( {s_{01} t_{10} } \right)u_{01} 
}{2}=(st)u
$$
$$
\frac{\left( {s_{10} t_{10} } \right)u_{01} -\left( 
{s_{01} t_{10} } \right)u_{01} }{2}=0
$$
$$\frac{\left( {s_{10} t_{00} } 
\right)u_{00} +\left( {s_{01} t_{00} } \right)u_{00} }{2}=(st)u
$$ 
$$
\frac{\left( {s_{10} t_{00} } \right)u_{00} -\left( {s_{01} t_{00} } 
\right)u_{00} }{2}=0.
$$
Hence $P_k (s,t,u)=\sum\limits_{l=0}^7 {\left[ {\pi 
_l \left( {(st)u} \right)} \right]} ^2W_t$. Using Corollary \ref{coro}, we obtain 
{\scriptsize
\[
P_k (1,1,1)=P_k (1,i_1 ,i_1 )=P_k (i_1 ,1,i_1 )=P_k (i_1 ,i_1 ,1)=P_k (i_2 
,i_5 ,i_3 )=P_k (i_2 ,i_6 ,i_7 )=P_k (i_4 ,i_6 ,i_3 )=P_k (i_4 ,i_5 ,i_7 )
\]
\[
P_k (i_1 ,1,1)=P_k (1,1,i_1 )=P_k (1,i_1 ,1)=P_k (i_1 ,i_1 ,i_1 )=P_k (i_2 
,i_5 ,i_7 )=P_k (i_2 ,i_6 ,i_3 )=P_k (i_4 ,i_6 ,i_7 )=P_k (i_4 ,i_5 ,i_3 )
\]
\[
P_k (i_2 ,1,1)=P_k (1,i_5 ,i_3 )=P_k (1,i_6 ,i_7 )=P_k (i_1 ,i_5 ,i_7 )=P_k 
(i_1 ,i_6 ,i_3 )=P_k (i_4 ,1,i_1 )=P_k (i_2 ,i_1 ,i_1 )=P_k (i_4 ,i_1 ,1)
\]
\[
P_k (1,1,i_3 )=P_k (1,i_1 ,i_7 )=P_k (i_1 ,1,i_7 )=P_k (i_1 ,i_1 ,i_3 )=P_k 
(i_2 ,i_5 ,1)=P_k (i_2 ,i_6 ,i_1 )=P_k (i_4 ,i_5 ,i_1 )=P_k (i_4 ,i_6 ,1)
\]
\[
P_k (i_4 ,1,1)=P_k (1,i_5 ,i_7 )=P_k (1,i_6 ,i_3 )=P_k (i_1 ,i_5 ,i_3 )=P_k 
(i_1 ,i_6 ,i_7 )=P_k (i_2 ,1,i_1 )=P_k (i_2 ,i_1 ,1)=P_k (i_4 ,i_1 ,i_1 )
\]
\[
P_k (1,i_5 ,1)=P_k (1,i_6 ,i_1 )=P_k (i_1 ,i_5 ,i_1 )=P_k (i_1 ,i_6 ,1)=P_k 
(i_2 ,1,i_3 )=P_k (i_2 ,i_1 ,i_7 )=P_k (i_4 ,1,i_7 )=P_k (i_4 ,i_1 ,i_3 )
\]
\[
P_k (1,i_6 ,1)=P_k (1,i_5 ,i_1 )=P_k (i_1 ,i_5 ,1)=P_k (i_1 ,i_6 ,i_1 )=P_k 
(i_2 ,1,i_7 )=P_k (i_2 ,i_1 ,i_3 )=P_k (i_4 ,1,i_3 )=P_k (i_4 ,i_1 ,i_7 )
\]
\[
P_k (1,1,i_7 )=P_k (1,i_1 ,i_3 )=P_k (i_1 ,1,i_3 )=P_k (i_1 ,i_1 ,i_7 )=P_k 
(i_2 ,i_5 ,i_1 )=P_k (i_2 ,i_6 ,1)=P_k (i_4 ,i_5 ,1)=P_k (i_4 ,i_6 ,i_3 )
\]}
%\normalsize{
Therefore, the expected payoff to player $k$ can be rewritten as
\begin{eqnarray*}
\sum _k (\sigma ,\tau ,\upsilon )&=& \frac{1}{64}[8P_k (1,1,1)+8P_k 
(i_1 ,1,1)+8P_k (i_2 ,1,1)+8P_k (1,1,i_3 )\\
&+& 8P_k (i_4 ,1,1)+8P_k (1,i_5,1)+8P_k (1,i_6 ,1)+8P_k (1,1,i_7 )]\\ \\
%&=\frac{1}{8}[ {P_k (1,1,1)+P_k (i_1,1,1)+P_k (i_2 ,1,1)
%+P_k (1,1,i_3 )+P_k (i_4 ,1,1)+P_k (1,i_5 ,1)
%+P_k (1,i_6 ,1)+P_k (1,1,i_7 )}] 
%&=\frac{1}{8}&[ {1\cdot W_0 +1\cdot W_1 
%+1\cdot W_2 +1\cdot W_3 +1\cdot W_4 +1\cdot W_5 +1\cdot W_6 +1\cdot W_7 }] \\ 
&=& \frac{W_0 +W_1 +W_2 +W_3 +W_4 +W_5 +W_6 
+W_7 }{8}
\end{eqnarray*}
Note this the average of the payoffs for player $k$.

\begin{theorem}{\rm 
The strategic profile $(\sigma, \tau, \upsilon )$ is a Nash equilibrium.}
\end{theorem}

\begin{proof} 
We can consider two cases.

\noindent CASE 1: $\tau=t=t_0 +t_1 i_1 +t_2 i_5 +t_3 
i_6 $ is a pure quantum strategy, where the $t_{k}$'s are real numbers with $t_0 ^2+t_1 ^2+t_2 ^2+t_3 
^2=1$. Then the expected payoff to player 2 is given by
\begin{eqnarray*}
P_2 (\sigma, t,\upsilon)&=& \frac{1}{16}
P_2 (1,t,1)+P_2 (1,t,i_1 )+P_2 (1,t,i_3 )+P_2 (1,t,i_7 )+P_2 (i_1 ,t,1)\\
&+& P_2(i_1 ,t,i_1 )+P_2 (i_1 ,t,i_3 )+P_2 (i_1 ,t,i_7 )+ P_2 (i_2 ,t,1)+P_2 (i_2 ,t,i_1)\\
&+& P_2 (i_2 ,t,i_3 )+P_2 (i_2 ,t,i_7 )+P_2(i_4 ,t,1)+P_2 (i_4 ,t,i_1)+P_2 (i_4 ,t,i_3 )\\
&+& P_2 (i_4 ,t,i_7 )
\end{eqnarray*}
By Corollary \ref{coro}, we obtain
\begin{eqnarray*}
 P_2 (\sigma,t,\upsilon )&=& \frac{1}{16}
 \sum\limits_{k=0}^7 [ \pi _k \left( (1t)1 \right)]^2Y_k 
+\sum\limits_{k=0}^7 [ \pi _k \left( (1t)i_1  \right)]^2Y_k 
+\sum\limits_{k=0}^7 [ \pi _k \left( (1t)i_3  \right)]^2Y_k \\
&+& \sum\limits_{k=0}^7 [ \pi _k \left( (1t)i_7 \right)]^2Y_k 
 +\sum\limits_{k=0}^7 [ \pi _k \left( (i_1 t)1 \right)]^2 Y_k 
 +\sum\limits_{k=0}^7 [ \pi _k \left( (i_1 t)i_1 \right)]^2Y_k\\
  &+& \sum\limits_{k=0}^7 [ \pi _k \left( (i_1 t)i_3\right) ]^2Y_k 
  +\sum\limits_{k=0}^7 [ \pi _k \left( (i_1t)i_7  \right) ]^2Y_k 
 +\sum\limits_{k=0}^7 [ \pi _k \left( (i_2 t)1 \right)]^2Y_k \\
 &+& \sum\limits_{k=0}^7 [ \pi _k \left( (i_2 t)i_1\right)]^2Y_k 
 +\sum\limits_{k=0}^7 [ \pi _2 \left( (i_1 t)i_3 \right)]^2Y_k 
 +\sum\limits_{k=0}^7 [ \pi _2 \left((i_1 t)i_7 \right) ]^2Y_k \\ 
 &+& \sum\limits_{k=0}^7 [ \pi _k \left( (i_4 t)1 \right) ]^2Y_k 
 +\sum\limits_{k=0}^7 [ \pi _k \left( (i_4 t)i_1  \right)]^2Y_k 
 +\sum\limits_{k=0}^7 [ \pi _k \left( (i_4 t)i_3\right)]^2Y_k \\
 &+& \sum\limits_{k=0}^7 [ \pi _k \left( (i_4t)i_7  \right) ]^2Y_k
 \end{eqnarray*}
or equivalently \begin{eqnarray*}
P_2 (\sigma,t,\upsilon )&=& \frac{1}{16}\left(t_0 ^2Y_0 +t_1 ^2Y_1 +t_2 ^2Y_5 +t_3 ^2Y_6 \right)+\left( t_1^2Y_0 +t_0 ^2Y_1 +t_3 ^2Y_5 +t_2 ^2Y_6  \right)\\
&+& \left( t_0 ^2Y_3 +t_1^2Y_7 +t_2 ^2Y_2 +t_3 ^2Y_4  \right)+\left( t_1 ^2Y_3 +t_0 ^2Y_7 +t_3 ^2Y_2 +t_2 ^2Y_4  \right)\\
 &+& \left( t_1^2Y_0 +t_0 ^2Y_1 +t_3 ^2Y_5 +t_2 ^2Y_6  \right)+\left( t_0 ^2Y_0 +t_1^2Y_1 +t_2 ^2Y_5 +t_3 ^2Y_6 \right) \\
 &+& \left( t_1 ^2Y_3 +t_0 ^2Y_7 +t_3 ^2Y_2 +t_2 ^2Y_4 \right)+\left( t_0 ^2Y_3 +t_1 ^2Y_7 +t_2 ^2Y_2 +t_3 ^2Y_4 \right)\\
 &+& \left( t_2 ^2Y_3 +t_3^2Y_7 +t_0 ^2Y_2 +t_1 ^2Y_4  \right)+\left( t_3 ^2Y_3 +t_2 ^2Y_7 +t_1 ^2Y_2 +t_0 ^2Y_4  \right)\\
 &+& \left( t_2^2Y_0 +t_3 ^2Y_1 +t_0 ^2Y_5 +t_1 ^2Y_6  \right)+\left( t_3 ^2Y_0 +t_2^2Y_1 +t_1 ^2Y_5 +t_0 ^2Y_6 \right)\\
 &+& \left( t_3 ^2Y_3 +t_2 ^2Y_7 +t_1 ^2Y_2 +t_0 ^2Y_4  \right)+\left( t_2^2Y_3 +t_3 ^2Y_7 +t_0 ^2Y_2 +t_1 ^2Y_4 \right)\\
 &+& \left( t_3 ^2Y_0 +t_2^2Y_1 +t_1 ^2Y_5 +t_0 ^2Y_6  \right)+\left( t_2 ^2Y_0 +t_3 ^2Y_1 +t_0 ^2Y_5 +t_1 ^2Y_6 \right)
\end{eqnarray*}
Simplifying gives,
\begin{align*}
P_2 (\sigma,t,\upsilon )&=2Y_0 \left( t_0 ^2+t_1 ^2+t_2 ^2+t_3 ^2 \right)+2Y_1 \left( t_0 ^2+t_1^2+t_2 ^2+t_3 ^2 \right)\\
&+2Y_2 \left( t_0 ^2+t_1 ^2+t_2 ^2+t_3 ^2\right)+2Y_3 \left( t_0 ^2+t_1 ^2+t_2 ^2+t_3 ^2 \right) \\ 
&+2Y_4 \left( t_0 ^2+t_1 ^2+t_2 ^2+t_3 ^2 \right)+2Y_5 \left( t_0 ^2+t_1^2+t_2 ^2+t_3 ^2 \right) \\
&+2Y_6 \left( t_0 ^2+t_1 ^2+t_2 ^2+t_3 ^2\right)+2Y_7 \left( t_0 ^2+t_1 ^2+t_2 ^2+t_3 ^2 \right) \\ \\
&=\frac{Y_0 +Y_1 +Y_2 +Y_3 +Y_4 +Y_5 +Y_6 +Y_7 }{8}
\end{align*} 
Hence, player 2 is indifferent between his pure quantum strategies.

\noindent CASE 2: Player 2 employs the mixed quantum strategy $\mu$ which is a 
probability distribution over $S^{3}$. Then the expected payoff to Player 2
is given by
\[
\Sigma (\sigma,\mu,\upsilon)=\int\limits_{S^3\times S^3\times S^3} 
{P_2 (s,t,u)d(\sigma \times \mu \times \upsilon )(s,t,u)} 
\]
Applying Fubini's Theorem, we obtain
\begin{align*}
 \Sigma (\sigma, \mu, \upsilon )&=\int\limits_{S^3\times S^3\times S^3} 
{P_2 (s,t,u)d(\sigma \times \mu \times \upsilon )s,t,u)} \\
&=\int\limits_{S^3} {\left[ {\int\limits_{S^3\times S^3} {P_2 
(s,t,u)d(\sigma \times \upsilon )}(s,u)} \right]d} \mu (t) \\
&=\int\limits_{S^3} 
{\left( {\frac{1}{8}\sum\limits_{k=0}^7 {Y_k } } \right)}\mu (t)\\
&=\frac{1}{8}\sum\limits_{k=0}^7 
{Y_k } \mu \left( {S^3} \right)=\frac{1}{8}\sum\limits_{k=0}^7 
{Y_k }
\end{align*}

Hence, Player II is indifferent between all his/her mixed quantum 
strategies. Now, if we interchange players, we get, by symmetry, the same 
result. Therefore the special discrete distribution is a Nash equilibrium 
with expected payoff to the players 
$$
\frac{1}{8}\left( {\sum\limits_{k=0}^7 
{X_k ,\;\sum\limits_{k=0}^7 {Y_k ,\;\sum\limits_{k=0}^7 {Z_k} } } }
\right).
$$
\end{proof}

\section{Applications} 

We give two straightforward applications, one to a zero-sum game, the other 
to a dilemma game which is not a zero-sum game.

For our zero-sum game we consider the final stage of the Nash-Shapley Poker 
Model [Binmore]. This final strategic form is a $3 \times 2$ zero-sum game with 
payoff function given by the tables below, where we denote Player 1's strategy 
space by $\{s_1,s_2 \}$, Player 2's strategy space by $\{t_1,t_2 \}$, 
and Player 3's strategy space by $\{u_1,u_2\}$.

\begin{table}[h]
  \begin{minipage}{2.5in}
  \begin{tabular}{|c|c|c|}
	  \hline
	    &$t_1$&$t_2$\\
		  \hline
      $s_1$&$(-2,-2,4)$&$(-2,6,-4)$\\
      \hline
	     $s_2$&$(6,-2,-4)$&$(10,10,20)$\\
			\hline
	  \end{tabular} \\ \\
	  \centering 
	  $u_1$
  \end{minipage}
  \begin{minipage}{2.5in}
      \begin{tabular}{|r|r|r|}
	  	  \hline
	    &$t_1$&$t_2$\\
		  \hline
      $s_1$&$(0,0,0)$&$(2,-4,2)$\\
      \hline
			$s_2$&$(-4,2,0)$&$(-3,-3,6)$\\
			\hline
	  \end{tabular}\\ \\
	  \centering 
	  $u_2$
  \end{minipage}
  \caption{\small{Nash-Shapely poker payoff function. Table on the left is the payoff function when player 3 play's $u_1$, while the table on the right is the payoff function when player 3 employ's $u_2$.}}
 \end{table}

There is no classical pure strategy equilibrium. But there is a unique 
classical mixed strategy equilibrium where player 1 uses his/her second 
strategy with probability $p=\sqrt {\frac{7}{5}} -1\approx 0.18$, player 2
uses his/her second strategy with probability $q=\sqrt {\frac{7}{5}} 
-1\approx 0.18$, and player 3 uses his/her second strategy with 
probability$r=\frac{4p+8}{5p+12}\approx 0.68$ with expected payoff to the 
players $\left( {-0.40456,\;-0.40456,\;0.80912} \right)$. So quantizing this 
$3\times2$ game as above and applying our theorem we have a mixed quantum strategy 
equilibrium given by each player utilizing their special discrete 
distribution with payoffs given by $\left( {0.875,\;0.875,\;-1.75} \right)$. 
We note that in the classical game, the third player has a distinct 
advantage but this advantage disappears in the quantized version. 

For our non-zero sum example, consider the three player dilemma game 
examined by [BH: Benjamin and Hayden]. In [BH], they consider an EWL 
quantization trough a different initial state than ours. The payoff function 
is given by the below tables, where players have the same strategy space 
denoted by$\{C,D\}$.

\begin{table}[h]
  \begin{minipage}{2.5in}
  \begin{tabular}{|c|c|c|}
	  \hline
	    &$C$&$D$\\
		  \hline
      $C$&$(-2,-2,4)$&$(-2,6,-4)$\\
      \hline
	     $D$&$(6,-2,-4)$&$(10,10,20)$\\
			\hline
	  \end{tabular} \\ \\
	  \centering 
	  $C$
  \end{minipage}
  \begin{minipage}{2.5in}
      \begin{tabular}{|r|r|r|}
	  	  \hline
	    &$C$&$D$\\
		  \hline
      $C$&$(0,0,0)$&$(2,-4,2)$\\
      \hline
			$D$&$(-4,2,0)$&$(-3,-3,6)$\\
			\hline
	  \end{tabular}\\ \\
	  \centering 
	  $D$
  \end{minipage}
  \caption{\small{Three player Prisoner's Dilemma.}}
 \end{table}

There is a unique classical pure strategy equilibrium \textit{(D, D, D)} with payoff to the 
players (2, 2, 2). So quantizing this 3x2 game as above and applying our 
theorem we have a mixed quantum strategy equilibrium given by each player 
utilizing their special discrete distribution with payoffs given by (.5, .5, 
.5). We note that in the quantized game, the players get lower payoffs than 
the ones they get in the classical version when they employ the special 
discrete distribution.

%\end{document}


==> Chapter71.tex <==
\chapter{Properly Quantizing History Dependent Parrondo Games}

The Bleiler formalism for quantum mixing discussed in chapter 3 inspires a paradigm for game quanitzation that is proper by construction. This paradigm, which will be referred to as the Bleiler quantization paradigm, in fact produces the EWL protocol as a special case. The Bleiler quantization paradigm is reviewed in this chapter and an application leading to a proper quanitzation of the history dependent (HD) Parrondo games is discussed.

\section{Bleiler Quantization Paradigm}

Description of the joint state space of the qubits is parametrized by the observational basis $\left\{\ket{0}, \ket{1}\right\}$. However, fundamental to the construction of the Bleiler quanitzation paradigm is a different basis of the joint state space, the so-called action basis given as follows. Fix an initial state on the observational basis. In the following discussion the initial state $I=\frac{1}{\sqrt 2}\left(\ket{00 \dots 0}+\ket{11 \dots 1}\right)$ is used, adjusted appropriately for the number of qubits being utilized.

Consider the qubits as having embedded the classical actions of ``No Flip'' ($N$) and ``Flip'' ($F$). That is, for a given initial state of a qubit in the observational basis, the action $N$ corresponds to the state staying unchanged while the action $F$ corresponds to a change in the state. Moreover, these classical actions are embedded into the collection of actions on the qubits, namely $SU(2)$, such that the collection of action profiles on our qubits, when applied to $I$, give a basis for the joint state space of the qubits. 

For example, for three qubits, we have 
$$
I=\frac{1}{\sqrt 2}\left(\ket{000}+\ket{111}\right)
$$
and 
$$
N=\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill \\
 0 \hfill & 1 \hfill \\
\end{array} }} \right), \quad
F=\left( {{\begin{array}{*{20}c}
 0 \hfill &  {-\bar {\eta }}  \hfill \\
 \eta  \hfill & 0 \hfill \\
\end{array} }} \right)
$$
where $\eta \in U(1)$ is chosen such that the eight outcome states of our 
game 
$$
\mathcal{B}_{NF}=\left\{\ket{NNN}, \ket{NNF}, \ket{NFN}, \ket{NFF}, \ket{FNN}, \ket{FNF}, \ket{FFN}, \ket{FFF}\right\}
$$
form an orthogonal basis of the state 
space $\mathbb{C}^8$ which carries the observational basis 
$$
\mathcal{B}=\left\{ {\left| {000} \right\rangle 
,\left| {001} \right\rangle ,\left| {010} \right\rangle ,\left| {011} 
\right\rangle ,\left| {100} \right\rangle ,\left| {101} \right\rangle 
,\left| {110} \right\rangle ,\left| {111} \right\rangle } \right\}.
$$
Note that $F\left|0\right\rangle=\eta\left|1\right\rangle$ and $F\left|1\right\rangle=-\bar{\eta}\left|0\right\rangle$.
The relationship between $\mathcal{B}$ and $\mathcal{B}_{FN}$ is made explicit by studying how the eight different combinations of the classical $N$ and $F$ act on the initial state $I$. 
\begin{equation}\label{NNN}
NNN(I)=\frac{1}{\sqrt 2}\left(\ket{000}+\ket{111}\right)=I
\end{equation}
\begin{equation}\label{NNF}
NNF(I)=\frac{1}{\sqrt 2}\left(\ket{00(\eta1)}+\ket{11(-\bar{\eta}0)}\right)
\end{equation}
\begin{equation}\label{NFN}
NFN(I)=\frac{1}{\sqrt 2}\left(\ket{0(\eta1)0}+\ket{1(-\bar{\eta}0)1}\right)
\end{equation}
\begin{equation}\label{NFF}
NFF(I)=\frac{1}{\sqrt 2}\left(\ket{0(\eta1)(\eta1)}+\ket{1(-\bar{\eta}0)(-\bar{\eta}0)}\right)
\end{equation}
\begin{equation}\label{FNN}
FNN(I)=\frac{1}{\sqrt 2}\left(\ket{(\eta1)00}+\ket{(-\bar{\eta}0)11}\right)
\end{equation}
\begin{equation}\label{FNF}
FNF(I)=\frac{1}{\sqrt 2}\left(\ket{(\eta1)0(\eta1)}+\ket{(-\bar{\eta}0)1(-\bar{\eta}0)}\right)
\end{equation}
\begin{equation}\label{FFN}
FFN(I)=\frac{1}{\sqrt 2}\left(\ket{(\eta1)(\eta1)0}+\ket{(-\bar{\eta}0)(-\bar{\eta}0)1}\right)
\end{equation}
\begin{equation}\label{FFF}
FFF(I)=\frac{1}{\sqrt 2}\left(\ket{(\eta1)(\eta1)(\eta1)}+\ket{(-\bar{\eta}0)(-\bar{\eta}0)(-\bar{\eta}0)}\right)
\end{equation}
%\[
%NNN(I)=\left( {{\begin{array}{*{20}c}
% 1 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 1 \hfill \\
%\end{array} }} \right),
%\quad
%NNF(I)=\left( {{\begin{array}{*{20}c}
% 0 \hfill \\
% {-\bar {\eta }} \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% \eta \hfill \\
% 0 \hfill \\
%\end{array} }} \right),
%\quad
%NFN(I)=\left( {{\begin{array}{*{20}c}
% 0 \hfill \\
% 0 \hfill \\
% {-\bar {\eta }} \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% \eta \hfill \\
% 0 \hfill \\
% 0 \hfill \\
%\end{array} }} \right),
%\quad
%NFF(I)=\left( {{\begin{array}{*{20}c}
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% {\bar {\eta }^2} \hfill \\
% {\eta ^2} \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
%\end{array} }} \right),
%\]
%\[
%FFF(I)=\left( {{\begin{array}{*{20}c}
% {\eta ^3} \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% {-\bar {\eta }^3} \hfill \\
%\end{array} }} \right),
%\quad
%FFN(I)=\left( {{\begin{array}{*{20}c}
% 0 \hfill \\
% {\eta ^2} \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% {\bar {\eta }^2} \hfill \\
% 0 \hfill \\
%\end{array} }} \right),
%\quad
%FNN(I)=\left( {{\begin{array}{*{20}c}
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% \eta \hfill \\
% {-\bar {\eta }} \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
%\end{array} }} \right),
%\quad
%FNF(I)=\left( {{\begin{array}{*{20}c}
% 0 \hfill \\
% 0 \hfill \\
% \eta^2 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
% \bar{\eta}^2 \hfill \\
% 0 \hfill \\
% 0 \hfill \\
%\end{array} }} \right)
%\]
The value of $\eta$ that ensure the orthogonality of $\mathcal{B}_{NF}$ is computed from the 
non-trivial orthogonality conditions that follow from equations \ref{NNN}-\ref{FFF}.
\[
\left\langle {NNN(I),FFF(I)} \right\rangle =\eta^3-\bar{\eta} ^3=0
\]
\[
\left\langle {NNF(I),FFN(I)} \right\rangle =-\bar\eta }\cdot \bar {\eta }^2+\eta 
\cdot \eta ^2=-\bar {\eta }^3+\eta ^3=0,
\]
\[
\left\langle {NFN(I),FNF(I)} \right\rangle =-\bar {\eta }\cdot \bar {\eta }^2+\eta 
\cdot \eta ^2=-\bar {\eta }^3+\eta ^3=0,
\]
\[
\left\langle {NFF(I),FNN(I)} \right\rangle =\bar {\eta }^2\cdot \bar {\eta }+\eta 
^2\cdot (-\eta )=\bar {\eta }^3-\eta ^3=0
\]
Therefore $\eta ^6=1$ and $\eta =\frac{1}{2}+\frac{\sqrt 3 }{2}i$.

Write the right hand sides of equations \ref{NNN}-\ref{FFF} as vectors in $\mathbb{C}^8$ and use them as columns of the change of basis matrix $A$ that takes the action basis to the observational basis:
\[
A=\frac{1}{\sqrt 2}\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill 
& -\bar{\eta}^3 \hfill \\
 0 \hfill & \eta  \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 
\hfill & \bar{\eta}^2 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & \eta \hfill & 0 \hfill & 0 \hfill & \bar{\eta}^2 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & \eta^2 \hfill & -\bar{\eta} \hfill & 0 
\hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & \bar{\eta}^2 \hfill & \eta \hfill 
& 0 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & -\bar{\eta} \hfill & 0 \hfill & 0 \hfill & {\eta}^2 
\hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & -\bar{\eta} \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & {\eta}^2 \hfill & 0 \hfill \\
 1 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill 
& {\eta}^3 \hfill \\
\end{array} }} \right).
\]
This matrix is unitary by construction, so $\bar 
{A}^T=A^{-1}$ and the basis change matrix taking the 
observational basis to the action basis is
\[
A^{-1}=\left( {{\begin{array}{*{20}c}
 1 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill 
& 1 \hfill \\
 0 \hfill & \bar{\eta} \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 
-\eta \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & \bar{\eta} \hfill & 0 \hfill & 0 \hfill & -\eta \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & \bar{\eta ^2} \hfill & \eta^2 \hfill 
& 0 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & 0 \hfill & -\eta \hfill & \bar{\eta} \hfill & 
0 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & 0 \hfill & \eta^2 \hfill & 0 \hfill & 0 \hfill & \bar{\eta}^2 \hfill & 0 \hfill & 0 \hfill \\
 0 \hfill & \eta^2 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 
\hfill & \bar{\eta}^2 \hfill & 0 \hfill \\
 -\eta^3 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 \hfill & 0 
\hfill & 0 \hfill & \bar{\eta}^3 \hfill \\
\end{array} }} \right).
\]

The quantization will be proper if the classical HD Parrondo game is embedded in the quantization. To ensure this, following Flitney et al \cite{Flitney}, a quantum circuit known as a quantum multiplexer is employed. A quantum multiplexer is a sequence of multiply controlled one qubit gates, which are elements of $SU(2)$, that act on a target qubit under the control of the remaining qubits in the circuit.  The quantum multiplexer employed for the proper quantization of the HD Parrondo game here is given in Figure \ref{3qubitQM}. It targets the last qubit in the circuit with one of the gates $G_i$, where the choice of the particular $G_i$ is determined by the binary conficuration of the control qubits. The binary configuration is represented by the sequence of black and white circles, with a white circle representing the value $\ket{0}$ and a black circle representing the value $\ket{1}$.

\begin{figure}
\centerline{\includegraphics[scale=0.25]{3qubitQM.jpg}}
\caption{\small{Three qubit quantum multiplexer.}}
\label{3qubitQM}
\end{figure}

To represent the the biased coins as elements of $SU(2)$, consider them as superpositions of the actions of $N$ and $F$. In particular, if the classical coin is biased to show head with probability $p$, represent this coin as the $SU(2)$ element 
\begin{equation}\label{biased coin}
{\sqrt p}N+{\sqrt 1-p}F.
\end{equation}
Note that expression (\ref{biased coin}) is a quantum superposition and not a probabilistic combination. But when measured in the action basis, $N$ appears with probability $p$ and $F$ appears with probability $1-p$, faithfully reproducing the behavior of the classical coin. 

In fact, a partial ``inverse'' exists to this procedure which allows for the determination of a proabability bias on a coin from an element of $SU(2)$. Begin with a probability bias on a coin embedded into $SU(2)$ and from this determine a probability bias on a coin; this will give the original bias unchanged. Now begin with an arbitrary element of $SU(2)$ and produce a probabilistic bias on a coin from it, and then embed this bias back into $SU(2)$. There is no gaurantee that the original $SU(2)$ element will be obtained. 

The procedure is as follows. 


Whether the quantum game is winning or losing is determined by mimicking the classical situation. From the four $G_i \in SU(2)$, determine the classical Parrondo game given by the coin biases. Now proceed classically and establish the Markov process, compute the stable distribution $\pi_i$ over the histories, and embed this distribution as the action vector
\begin{equation}\label{vect in C8}
\left( 
\begin{array}{*{20}c}
 \sqrt{\pi_1} \hfill \\
 0 \hfill \\
 \sqrt{\pi_2} \hfill \\
 0 \hfill \\
 \sqrt{\pi_3} \hfill \\
 0 \hfill \\
 \sqrt{\pi_4} \hfill \\
 0 \hfill \\
\end{array} \right)
\begin{array}{*{20}c}
 {NNN} \hfill \\
 {NNF} \hfill \\
 {NFN} \hfill \\
 {NFF} \hfill \\
 {FNN} \hfill \\
 {FNF} \hfill \\
 {FFN} \hfill \\
 {FFF} \hfill \\
\end{array}
\end{array}
\end{equation}
and rewrite it in the observational basis and use the resulting vector as the initial state for the quantized HD Parrondo game. Apply the quantum multiplexer to this initial state and measure the output in the action basis. The result is a probability distribution over the action basis. Sum the probabilities 

Next we use the the Bleiler formalism to the quantization of a particular type of Parrondo game. Parrondo games are single player games in which the payoff to the player is the expectation. The games are of interest because they exhibit the \emph{Parrondo effect}; that is, when two or more games with negative expectation (losing game) are played in sequence, the resulting expectation to the player is positive. The game defined by the sequence is then referred to as the combined game and is called a winning game due to the positive expectation. Parrondo et. al first formulated such games in \cite{Parrondo:99}. The subject of Parrondo games has seen much research activity since then. A comprehensive survey by Harmer and Abbott of Parrondo games and the Parrondo effect can be found in \cite{Harmer}.

Earlier work on the quantization of Parrondo games can be found in \cite{Meyer1}, where Meyer offers an analysis of the quantized capital dependent Parrondo game, and in \cite{Flitney:02}, where Flitney et. al propose quantizations of the history dependent (HD) Parrondo game. The main idea in both these papers is to first quantize the original game via a quantization protocol. The game sequences are then modeled by iterations of these protocols. At the end, a measurement is made and the expected payoff is computed from the resulting probability distribution. The relevant game theoretic question in this case is whether the quantization enhances or lowers the expected payoff. The Bleiler formalism shows that in case of the quantization of the HD Parrondo game, the answer is in the negative. 

\subsection{Capital Dependent Parrondo Games}\label{CDPG}

In \cite{Parrondo:99}, Parrondo et al describe two types of games which have the property that if individually repeated, the games result in a decreasing expected payoff to the player, yet when the two games are played in a deterministic or probabilistic sequence repeteadly, the expected payoff to the player is increases over time.

Suppose that $X(t)=0, 1, 2, \dots $ is the capital available to the player. If the player wins a game, then the capital increases by one, and if the player loses, then the capital decreases by one. The simplest type of this game, referred to in the literature as game $A$, is determined by a biased coin with probability of win $p$. That is, the capital increases by one with probability $p$ and decreases by one with probability $1-p$. Another game, called game $B$, is defined by two biased coins. The choice of which coin is to be played in an instance of the game is determined by the congureunce modulo 3 of the capital, $X(t)$, available to the player in that instance. Hence, game $B$ is defined by the rules given in table \ref{table:gameB}.

\begin{table}[ht]
\caption{Game B} % title of Table
\centering % used for centering table
\begin{tabular}{c c c} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
& Prob. of win & Prob. of loss \\ [0.5ex] % inserts table
%heading
\hline % inserts single horizontal line
$X(t)\equiv 0 \hspace{.05in} \mbox{mod} \hspace{.05in} 3$  &$p_{1}$ & $1-p_1$ \\ % inserting body of the table
$X(t)\equiv 1 \hspace{.05in} {\rm or} \hspace{.05in} 2 \hspace{.05in} \mbox{mod} \hspace{.05in} 3$ & $p_{2}$ & $1-p_2$ \\[1ex] % [1ex] adds vertical space
\hline %inserts single line
\end{tabular}
\label{table:gameB} % is used to refer this table in the text
\end{table}

Parrondo et al set $p=\frac{1}{2}-\epsilon$, $p_1=\frac{1}{10}-\epsilon$, $p_2=\frac{3}{4}-\epsilon$, for $\epsilon >0$ as an example of games $A$ and $B$ which have the tendency to be losing if played individually in a sequence, but which, when combined in a randomly alternating sequence, have a tendency to win. By ``tendency" is meant the long term behavior of the capital $X(t)$, which for a game with tendency to lose if a decreasing function of time, and for a game with tendency to win is an increasing function of time. For a game with a tendency to be fair, $X(t)$ will remain constant over time. Both games can in fact be made losing, winning, or fair by choosing $\epsilon >0$, $\epsilon < 0$ and $\epsilon = 0$, respectively. Parrondo et al consider in detail the case when both games $A$ and $B$ are fair. Game $B$ is analyzed as the Markov process $Y(t) \equiv X(t)$ (mod 3). The transition matrix for game $B$ is

\begin{equation}\label{tran gameB}
T=\left(\begin{array}{ccc}
0 & \frac{1}{4} & \frac{3}{4} \\ \\
\frac{1}{10} & 0 & \frac{1}{4}\\ \\
\frac{9}{10} & \frac{3}{4} & 0
\end{array}\right).
\end{equation}

\noindent The stationary state for this Markov process can be computed from the matrix equation

\begin{equation}\label{matrix eq}
\left(\begin{array}{ccc}
0 & \frac{1}{4} & \frac{3}{4} \\ \\
\frac{1}{10} & 0 & \frac{1}{4}\\ \\
\frac{9}{10} & \frac{3}{4} & 0
\end{array}\right)
\left(\begin{array}{c}
\pi_0 \\ \\ \pi_1 \\ \\ \pi_2
\end{array}\right)
=
\left(\begin{array}{c}
\pi_0 \\ \\ \pi_1\\ \\ \pi_2
\end{array}\right)
\end{equation}

\noindent where $\pi_i$ is the probability of the capital $X(t)$ taking on a values congruent to $i$ (mod 3). The matrix equation \ref{matrix eq} gives rise to the following system of equations

\begin{align}
\frac{1}{4}\pi_2	+ \frac{3}{4}\pi_3 = \pi_1\\
\frac{1}{10}\pi_1	+ \frac{1}{4}\pi_3 = \pi_2\\
\frac{9}{10}\pi_1	+ \frac{3}{4}\pi_2 = \pi_3
\end{align}

\noindent which has the following solution.
$$
\pi_1=\pi_1, \quad \pi_2=\frac{2}{5}\pi_1, \quad \pi_3=\frac{6}{5}\pi_1.
$$

\noindent Since the game is assumed to be fair, $p_1\pi_0+p_2\pi_1+p_2\pi_2=\frac{1}{2}$, and one computes $\pi_0=\frac{5}{13}$, $\pi_1=\frac{2}{13}$, $\pi_2=\frac{6}{13}$. 

Now if the fair games $A$ and $B$ are played with equal probability, the resulting capital is an increasing function. To see this, let $q$ be the probability with which the game $A$ is played. Then game $B$ is played with probability $(1-q)$. Again, we analyze the Markov sequence $Y(t) \equiv X(t)$ (mod 3), but this time the transition matrix is 

\begin{equation}\label{matrix eq alternating generic}
T'=\left(\begin{array}{ccc}
0 & \frac{1}{2}q+\frac{1}{4}(1-q) & \frac{1}{2}q+\frac{3}{4}(1-q) \\ \\
\frac{1}{2}q+\frac{1}{10}(1-q) & 0 & \frac{1}{2}q+\frac{1}{4}(1-q)\\ \\
\frac{1}{2}q+\frac{9}{10}(1-q) & \frac{1}{2}q+\frac{3}{4}(1-q) & 0
\end{array}\right)
\end{equation}

\noindent Set $q=\frac{1}{2}$ to get 

\begin{equation}\label{matrix eq alternating}
T'=\left(\begin{array}{ccc}
0 & \frac{1}{4}+\frac{1}{8} & \frac{1}{4}+\frac{3}{8} \\ \\
\frac{1}{4}+\frac{1}{20} & 0 & \frac{1}{4}+\frac{1}{8}\\ \\
\frac{1}{4}+\frac{9}{20} & \frac{1}{4}+\frac{3}{8} & 0
\end{array}\right)
=
\left(\begin{array}{ccc}
0 & \frac{3}{8} & \frac{5}{8} \\ \\
\frac{3}{10} & 0 & \frac{3}{8}\\ \\
\frac{7}{10} & \frac{5}{8} & 0
\end{array}\right)
\end{equation}

Computing the stationary state $(\pi'_0, \pi'_1, \pi'_2)^T$ for the case in which the game is fair gives $\pi'_=\frac{245}{709}$, $\pi'_1=\frac{180}{709}$, and $\pi'_2=\frac{284}{709}$ upto the normalization constant. Note that this mixed game is no longer fair because $\pi'_0=\frac{245}{709}=0.346$ is closer to $\frac{1}{3}$ than $\pi_0=0.385$ 

\subsection{History Dependent Parrondo Game}
The history dependent (HD) Parrondo game, introduced in \cite{Parrondo:99} by Parrondo et al, is a one player biased coin flipping game, where the choice of the biased coin depends on the history of the game. A history dependent Parrondo game $B$ with two historical steps is reproduced here in the following table. 

\begin{center}$B:$
\begin{tabular}{c|c|c|c|c}
 Before last & Last& Coin & Prob. of win & Prob. of loss \\
$t-2$        & $t-1$& ~ & at $t$ & at $t$ \\\hline
loss & loss & $B_1'$ & $p_1$ & $1-p_1$\\ loss & win & $B_2'$ & $p_2$
& $1-p_2$ \\ win & loss & $B_3'$ & $p_3$ & $1-p_3$ \\ win & win &
$B_4'$ & $p_4$ & $1-p_4$ \\
\end{tabular}
\end{center}

Let $X(t)$ be the capital available to the player at time $t$ which goes up or down by one unit depending on whether the player wins or loses the game, respectively. Setting up the Markov process 
$$
Y(t)=\left(\begin{array}{c}
X(t)-X(t-1) \\ X(t-1)-X(t-2)
\end{array}\right)
$$
allows one to analyze the long term behavior of the capital in the game $B$ via the stationary state of the process $Y(t)$. The transition matrix for this process is 
$$
\left(\begin{array}{cccc}
1-p_1 & 0 & 1-p_3 & 0 \\  p_1 & 0 & p_3 & 0 \\ 0 & 1-p_2 & 0 & 1-p_4 \\ 0 & p_2 & 0 & p_4 
\end{array}\right)
$$
The stationary state can be computed from the following equations
$$
(1-p_1)v_1+(1-p_3)v_3=v_1
$$
$$
p_1v_1+p_3v_3=v_2
$$
$$
(1-p_2)v_2+(1-p_4)v_4=v_3
$$
$$
p_2v_2+p_4v_4=v_4
$$
and is given by 
$$
\left(\begin{array}{c}
v_1 \\ v_2 \\v_3 \\v_4 
\end{array}\right)=\frac{1}{N}\left(\begin{array}{c}
(1-p_3)(1-p_4) \\ p_1(1-p_4) \\ p_1(1-p_4) \\ p_1p_2
\end{array}\right)
$$
after setting the free variable $v_4=p_1p_2$, and $N$ is the normalization constant equaling
$$
\sqrt{\left[(1-p_3)(1-p_4)\right]^2+2\left[(1-p_4)p_1\right]^2+(p_1p_2)^2}
$$
which upon simplification and because of the equivalence of the $2$-norm and the $1$-norm of vectors simplifies to 
$$ 
N=(1-p_4)(2p_1+1-p_3)+p_1p_2
$$ 

Consequently, the probability of winning in a generic run of the game $B$ is 

\begin{equation}\label{p of win}
p_{\rm win}=\sum_{j=1}^{4}\pi_{st,j}p_{j}=\frac{p_1\left(p_2+1-p_4\right)}{\left(1-p_4\right)\left(2p_1+1-p_3\right)+p_1p_2}
\end{equation}

\noindent where $\pi_{st,j}$ is the probability that a certain history $j$, represented in binary format, will occur, while $p_{j}$ is the probability of win upon the flip of the third coin corresponding to history $j$. This can be rewritten as $p_{\rm win} =1/(2+c/s)$, with
$s=p_1(p_2+1-p_4)>0$ for any choice of the rules, and
$c=(1-p_4)(1-p_3)-p_1p_2.$ Therefore, game $B$ obeys the following
rule: if $c < 0$, $B$ is winning or has positive expected payoff; if $c= 0$, $B$ is
fair; and if $c> 0$, $B$ is losing or has negative expected payoff. 

The authors of \cite{Kay:03} and \cite{Parrondo:99} show the remarkable result that a random or deterministic sequence of Parrondo games of type $A$ and/or $B$ in which the individual games are biased toward losing, can be made winning. An analysis of the values of the probabilities $p$ for a game of type $A$ and probabilities $p_{i}, 1\leq i \leq 4$ for a game of type $B$ determines the {\it Parrondo region}, a region inside the unit hypercube in which the Parrondo effect manifests itself. %A sequential play of Parrondo games of type $A$ and $B$ or just of game $B$ exhibits the {\it Parrondo effect} if when played individually, the two games give a negative expected payoff, but a periodic or random play of the two games leads to a positive expected payoff. 
%
%\subsection{Quantization of HD Parrondo Games}
%
%In \cite{Flitney:02}, Flitney et. al quantize the type $A$ Parrondo game by the action of an element of $SU(2)$ on a qubit. This is equivalent to flipping a biased quantum coin. 
%
%The history dependent game with $(n-1)$ histories, is quantized with two different protocols. In both, $n$ qubits are required and the unitary operator is a $2^{n-1} \times 2^{n-1}$ block diagonal matrix with blocks composed of elements of $SU(2)$. In the language of quantum logic gates, this is a quantum multiplexer. The first $(n-1)$ qubits represent the history of the game, where $\ket{0}$ represent a loss and $\ket{1}$ represents a win. 
%
%The first protocol takes as the initial state any one of the basis states. Any one of these input states reproduces the classical HD Parrondo game with the appropriate history. For example, with initial state $\ket{00 \dots 0}$, the protocol reproduces the classical Parrondo game with history of loss in every one of the previous $(n-1)$ stages. This makes the protocol proper, but un-interesting since it does not enhance the expected payoff of the player. In other words, this quantization produces no results that the classical game cannot, and therefore offers no new game theoretic results. 
%
%The second protocol takes as input the initial state $\frac{1}{\sqrt{2}}\left(\left|00 \dots 0\right\rangle+\left|11 \dots 1\right\rangle\right)$.
%For a game with three histories, the initial state is $\frac{1}{\sqrt{2}}\left(\left|000\right\rangle+\left|111\right\rangle\right)$. With this initial state, the protocol indeed produces the results presented in \cite{Flitney:02}. But for these results to offer something new to game theory, the protocol must be proper, which it is not due to its inability to reproduce the classical game. That is, when played with the initial state $\frac{1}{\sqrt{2}}\left(\left|000\right\rangle+\left|111\right\rangle\right)$, the quantum HD Parrondo game assigns, upon measurement, a probability of $0$ to outcomes with histories $\ket{01}$ and $\ket{10}$ due to which the classical game cannot be reproduced. In the language of the Bleiler formalism, this quantization of the HD game fails to be proper. 
%
%When the quantum HD Parrondo game is combined via composition with the two games of type $A$ acting on the history qubits, all histories in the outcome state are assigned non-zero probabilities upon measurment. This allows for the possibility of reproducing the results of the classical sequence of two type $A$ games followed by the HD game for some choice of parameters of the quantization protocols for two games of type $A$ and the HD game. 
%
%In fact, it is entirely possible to reproduce the classical HD game from just the quantum HD game if the initial state is a seperable state but which is not a basis state. Details of this proper quantization follow. 
%
%\subsection{An Alternative Quantization of the History Dependent Parrondo Game}
%
%Following the authors of \cite{Flitney:02}, we restrict our attention to the details of the HD game with only 2 histories. The arbitrary case for $n-1$ histories can be got easily by generalization.
%
%The classical game is embedded in the quantized game via identification of outcomes of the classical game with the basis states of the complex projective Hilbert space $\mathbb{H}^{\otimes 3}$ of qubits. We fix the basis of $\mathbb{H}^{\otimes 3}$ to be the ordered computational basis 
%$$
%\mathcal{B}=\left\{ \ket{000}, \ket{001}, \ket{010}, \ket{011}, \ket{100}, \ket{101}, \ket{110}, \ket{111} \right\}
%$$
%%\begin{figure}\centerline{
%% \Qcircuit @C1em @R=.8em {
%%&\ctrlo{+1} &\qw &\ctrlo{+1} &\qw &\ctrl{+1} &\qw &\ctrl{+1} &\qw \\
%%  &\ctrlo{+1} &\qw &\ctrl{+1} &\qw &\ctrlo{+1} &\qw &\ctrl{+1} &\qw\\
%%  &\gate{g_0} &\qw &\gate{g_1} &\qw &\gate{g_2} &\qw &\gate{g_3} &\qw \\}}
%%\caption{\footnotesize{A quantum circuit representation of the block diagonal unitary operator used in the FNA protocol.}}
%%\label{3rd ord mult}
%%\end{figure}
%We take $\ket{0}$ to represent a loss and $\ket{1}$ to represent a win. The first two qubits in an element of $\mathcal{B}$ represent the history of the game, while the last qubit represents the outcome of at the present stage of the game.
%Consider the subset $\mathcal{W}=\left(\ket{001}, \ket{011}, \ket{101}, \ket{111}\right)$ of $\mathcal{B}$ in which the final qubit is always in the state $\ket{1}$. The elements of $\mathcal{W}$ represent a winning outcome in the classical game.
%
%As in the FNA, the matrix for the quantized HD Parrondo game is
%\begin{equation}\label{eqn:eq15}
%X=\left( {{\begin{array}{*{20}c}
% {X_1 } \hfill & 0 \hfill & 0 \hfill & 0 \hfill \\
% 0 \hfill & {X_2 } \hfill & 0 \hfill & 0 \hfill \\
% 0 \hfill & 0 \hfill & {X_3} \hfill & 0 \hfill \\
% 0 \hfill & 0 \hfill & 0 \hfill & {X_4 } \hfill \\
%\end{array} }} \right)
%\end{equation}
%with 
%\begin{equation}\label{eqn:eq16}
%X_{j}=\left( {{\begin{array}{*{20}c}
%a_j \hfil & b_j \hfill \\
%-\overline{b}_j \hfill & \overline{a}_j \hfill \\
%\end{array}} } \right)
%\end{equation}
%
%and $a_j, b_j \in \mathbb{C}$ satisfying $\left|a_j\right|^2+\left|b_j\right|^2=1$.
%
%However, unlike FNA, we take the initial state of three qubits to be un-entangled, say 
%\begin{equation}\label{unentangled state}
%\left|q_1q_2q_3\right\rangle= \left( {{\begin{array}{c}
%q_{11} \\
%q_{12} \\
%\end{array}} } \right) \otimes \left( {{\begin{array}{c}
%q_{21} \\
%q_{22} \\
%\end{array}} } \right) \otimes \left( {{\begin{array}{c}
%q_{31} \\
%q_{32} \\
%\end{array}} } \right);  \hspace{.2in} \left|q_{k1}\right|^2+\left|q_{k2}\right|^2=1; \hspace{.2in} k=1,2,3.
%\end{equation}
%
%We point out here that if the initial state of the qubits was the maximally entanglement state, then a single play of the quantum HD game will {\it not} preserve the classical game due to destruction of the histories of the game. The initial state may be written as a vector in $\mathbb{H}^{\otimes 3}$.
%\begin{equation}\label{vector form}
%\left|q_1q_2q_3\right\rangle= \left( {{\begin{array}{c}
%q_{11}q_{21}q_{31}\\
%q_{11}q_{21}q_{32}\\
%q_{11}q_{22}q_{31}\\
%q_{11}q_{22}q_{32}\\
%q_{12}q_{21}q_{31}\\
%q_{12}q_{21}q_{32}\\
%q_{12}q_{22}q_{31}\\ 
%q_{12}q_{22}q_{32}
%\end{array}} } \right); \hspace{.2in}  \sum_{r,s,t=1}^2\left|q_{1r}q_{2s}q_{3t}\right|^2=1
%\end{equation}
%
%The output from the quantum HD Parrondo game for the input state in expression (\ref{vector form}) is 
%
%\begin{equation}\label{output}
%\left|q_1q_2q_3\right\rangle= \left( {{\begin{array}{c}
%q_{11}q_{21}\left(a_1q_{31}+b_1q_{32}\right)\\
%q_{11}q_{21}\left(\overline{a}_1q_{32}-\overline{b}_1q_{31}\right)\\
%q_{11}q_{22}\left(a_2q_{31}+b_2q_{32}\right)\\
%q_{11}q_{22}\left(\overline{a}_2q_{32}-\overline{b}_2q_{31}\right)\\
%q_{12}q_{21}\left(a_3q_{31}+b_3q_{32}\right)\\
%q_{12}q_{21}\left(\overline{a}_3q_{32}-\overline{b}_3q_{31}\right)\\
%q_{12}q_{22}\left(a_4q_{31}+b_4q_{32}\right)\\ 
%q_{12}q_{22}\left(\overline{a}_4q_{32}-\overline{b}_4q_{31}\right)
%\end{array}} } \right) 
%\end{equation}
%
%with the normalizing condition taking the form
%\begin{eqnarray*}
%&\left|q_{11}\right|^2\left(\sum_{s=1}^2\left|q_{2s}\left(a_sq_{31}+b_sq_{32}\right)\right|^2+\left|q_{2s}\left(\overline{a}_sq_{32}-\overline{b}_sq_{31}\right)\right|^2\right) \\  &+\left|q_{12}\right|^2\left(\sum_{s=1}^2\left|q_{2s}\left(a_{s+2}q_{31}+b_{s+2}q_{32}\right)\right|^2+\left|q_{2s}\left(\overline{a}_{s+2}q_{32}-\overline{b}_{s+2}q_{31}\right)\right|^2\right)=1
%\end{eqnarray*} 
%
%Note that the output or final state in (\ref{output}) exhibits entanglement between the qubits. The probability of winning, $p_{\rm{win}}^Q$ is the sum of the amplitudes of the coefficients of the elements of $\mathcal{W}$ in (\ref{output}), namely,
%\begin{equation}\label{p of win}
%p_{\rm{win}}^{Q}=\left|q_{11}\right|^2\left(\sum_{s=1}^2\left|q_{2s}\right|^2\left|\overline{a}_sq_{32}-\overline{b}_sq_{31}\right|^2\right)+\left|q_{12}\right|^2\left(\sum_{s=1}^2\left|q_{2s}\right|^2\left|\overline{a}_{s+2}q_{32}-\overline{b}_{s+2}q_{31}\right|^2\right)
%\end{equation}  
%
%Switching to polar form of the complex numbers and using the conditions $\left|q_{k1}\right|^2+\left|q_{k2}\right|^2=\left|a_j\right|^2+\left|b_j\right|^2=1$ for all values of $j$ and $k$, we set
%\begin{equation}\label{polar qk1}
%q_{k1}=e^{i\phi_{q_{k}}}\cos\left(\frac{\theta_{q_{k}}}{2}\right)
%\end{equation}
%\begin{equation}\label{polar qk2}
%q_{k2}=e^{i\eta_{q_{k}}}\sin\left(\frac{\theta_{q_{k}}}{2}\right)
%\end{equation}
%
%\begin{equation}\label{aj}
%a_j= e^{i\phi_{j}}\cos\left(\frac{\theta_{j}}{2}\right)
%\end{equation}
%\begin{equation}\label{bj}
%b_j=e^{i\eta_{j}}\sin\left(\frac{\theta_{j}}{2}\right)
%\end{equation}
%
%with $\theta_{q_{k}},\theta_j \in \left[0,\pi\right]$, $\eta_{q_{k}},\eta_j, \phi_{q_{k}}, \phi_j \in \left[0,2\pi\right]$.  
%
%These substitutions allow us to reduce 
%\begin{equation}\label{mid term}
%\left|\overline{a}_jq_{32}-\overline{b}_jq_{31}\right|^2 =  \cos^2\left(\frac{\theta_j}{2}\right)\sin^2\theta_{q_{3}}+\sin^2\left(\frac{\theta_j}{2}\right)\cos^2\theta_{q_{3}}-2\Re\left\{a_j\overline{b}_jq_{31}\overline{q}_{32}\right\}
%\end{equation}
%
%with
%$$
%\Re\left\{a_j\overline{b}_jq_{31}\overline{q}_{32}\right\}=\cos\left(\theta_j-\eta_j+\phi_{q_{3}}-\eta_{q_{3}}\right)\cos\left(\frac{\theta_j}{2}\right)\sin\left(\frac{\theta_j}{2}\right)\cos\theta_{q_{3}}\sin\theta_{q_{3}}
%$$
%Substituting equations (\ref{polar qk1}) - (\ref{mid term}) into equation (\ref{p of win}) allows us to express $p_{\rm{win}}^Q$ in terms of {\it twenty one} real variables, each taking on values from the closed unit interval, versus only four such variable that express $p_{\rm{win}}$. 
%
%The expected payoff to the player in a single play of the classical HD Parrondo game is $2p_{\rm{win}}-1$ while in the quantum game it is $2p_{\rm{win}}^Q-1$. Quantization will enhance the payoff if $p_{\rm{win}}^Q > p_{\rm{win}}$. However, it is possible that for some range of values of some of the domain variables $p_{\rm{win}}^Q \leq p_{\rm{win}}$. In other words, the choice of initial state and the choice of the values of the phase variables in the unitary operator for the quantization lends the expected payoff a different behavior than the expected payoff in the classical game. 
%
%For example, consider the following case in which the initial state is the equal superposition
%\begin{equation}\label{equal super}
%\left( {{\begin{array}{c}
%\frac{1}{\sqrt{2}} \\
%\frac{1}{\sqrt{2}} \\
%\end{array}} } \right) \otimes 
%\left( {{\begin{array}{c}
%\frac{1}{\sqrt{2}} \\
%\frac{1}{\sqrt{2}} \\
%\end{array}} } \right) \otimes 
%\left( {{\begin{array}{c}
%\frac{1}{\sqrt{2}} \\
%\frac{1}{\sqrt{2}}\\
%\end{array}} } \right)=\frac{1}{\sqrt{8}}\left(1,1,1,1,1,1,1\right)^{T}.
%\end{equation}
%Then $p_{\rm{win}}^Q$ is simply
%
%\begin{equation}\label{eqn19}
%p_{\rm{win}}^{Q}=\frac{1}{8}\left(4-\sum_{j=1}^{4}\sin\theta_{j}\cos(\eta_j-\phi_j)\right)=\frac{1}{2}-\frac{1}{8}\sum_{j=1}^{4}\sin\theta_{j}\cos(\eta_j-\phi_j)
%\end{equation}
%
%For values of the phase angles $\eta_j, \phi_j$ such that $\sum_{j=1}^{4}\sin\theta_{j}\cos(\eta_j-\phi_j) >0$, the quantum game is losing. For values that satisfy $\sum_{j=1}^{4}\sin\theta_{j}\cos(\eta_j-\phi_j)<0$, the quantum game is winning, where as the game is fair when $\sum_{j=1}^{4}\sin\theta_{j}\cos(\eta_j-\phi_j) =0$.
%
%The simplest case to analyze is when $\eta_j=\phi_j$ since in this case 
%$$
%p_{\rm{win}}^{Q}=\frac{1}{2}-\frac{1}{8}\sum_{j=1}^{4}\sin\theta_{j}
%$$
%and is equal to $\frac{1}{2}$ for $\theta_j=0$ or $\theta_j=\pi$, meaning that the quantum game is fair. However, $p_{\rm{win}}^{Q}$ is equal to $\frac{1}{2}-\epsilon$, $\epsilon > 0$, for all other values of the $\theta_j$, meaning that the game is losing.

\section{Parrondo Effect in Quantum Games}

Flitney et. al model various sequences of quantum HD Parrondo game and the game of type $A$ as compositions of the quantum protocols, with ancilla qubits added to generate the history. However, this notion of ``sequences'' is also questionable when viewed from the perspective of the Bleiler formalism, for the formalism asserts that a quantizing a game not only requires the mention of a unitary operator from the state space to itself, but also requires an explicit mention of some initial state. This means that in a seqeuence of quantum Parrondo games of length $k$ played with some initial state, one can always reduce the sequence to the case where the last sub-game in the sequence is in fact {\it the} game with initial state equal to the output from the sequence of the last $(k-1)$ games. As such, the notion of a sequence of quantum HD Parrondo games is redundant, particularly if the sequence does not exhibit any form of Parrondo effect, which is the case with Flitney et. al's quantization of the HD Parrondo game. 

In fact, from this point of view, {\it any} unitary operator acting on some initial state of $n$ qubits may be viewed as a quantization protocol for a one player game $G$ with Im$G$ consisting of two possible outcomes, say ``win'' and ``lose''. This follows from the fact that once $\ket{0}$ is designated as representing loss and $\ket{1}$ as representing  win, the basis states of the state space of $n$ qubits partition into two disjoint sets: the set $\mathcal{L}$ of basis states with the last qubit equal to $\ket{0}$ forms the set of losing outcomes, while the set $\mathcal{W}$ consisting of basis states with the last qubit equal to $\ket{1}$ forms the set of winning outcomes. Identifying Im$G$ with $\left\{\mathcal{W},\mathcal{L}\right\}$ achieves the goal. The quantum game is described as winning if measurement of the final state produces a probability distribution over Im$G$ that results in a positive expectation, as losing if measurement of the final state produces a probability distribution over Im$G$ that results in a negative expectation, and as fair if measurement of the final state produces a probability distribution over Im$G$ that results in expectation equal to 0. 

Define a {\it winning state} to be a state that upon measurement produces a probability distribution over Im$G$ that gives a positive expectation. Similarly, define a {\it losing state} to be a state that upon measurement produces a probability distribution over Im$G$ that gives a negative expectation, and a {\it fair state} as a state that upon measurement produces a probability distribution over Im$G$ that gives a expectation of 0.

A Parrondo effect in quantum games can now characterized as the phenomenon that takes losing initial states to winning final states. The anti-Parrondo effect is the phenomenon that takes winning initial states to losing final states. That is, a quantum game exhibits the Parrondo effect if it takes losing states to winning states, and exhibits the anti-Parrondo effect if it takes winning states to losing states. This characterization of the Parrondo effect in terms of the initial state induces a three-way partitioning of the state space: $\mathcal{P}_L$, the set of all losing states, $\mathcal{P}_W$, the set of all winning state, and $\mathcal{P}_F$, the set of all fair states. The analysis of the Parrondo effect in quantum games now merely amounts to studying the dynamics of the elements of these partitions under the action of the quantum game.

As an example, consider the simplest case of one qubit, with the quantization protocol for a game $G$ with two possible outcomes given by the flip matrix 
$$
F=\left( {{\begin{array}{*{20}c}
 0 \hfill & 1 \hfill \\
 1 \hfill & 0 \hfill \\
\end{array} }} \right).
$$
Then clearly, the losing state $\ket{0}=(1,0)^{T} \in \mathcal{P}_L$ is sent to the winning state $\ket{1}=(0,1)^{T} \in \mathcal{P}_W$ and vice versa. The quantum game exhibits both the Parrondo and the anti-Parrondo effect!

Another interesting example is the Hadamard gate 
$$
H=\frac{1}{\sqrt 2 }\left( {{\begin{array}{*{20}c}
 1 \hfill & 1 \hfill \\
 1 \hfill & {-1} \hfill \\
\end{array} }} \right).
$$
as a quantization protocol for $G$. It takes the losing state $\ket{0}$ to the fair state $\frac{1}{\sqrt{2}}\left(\ket{0}+\ket{1}\right)$ and takes the winning state $\ket{1}$ to the fair state $\frac{1}{\sqrt{2}}\left(\ket{0}-\ket{1}\right)$. Moreover, applying the Hadamard to these fair states results in the losing state $\ket{0}$ and the winning state $\ket{1}$ respectively. Therefore, the square of the Hadamard gate, $H^2$, is a quantization protocol that sends a losing state to another losing state, and a winning state to a winning state. Quantum Parrondo effect thus defined holds the potential to raise interesting questions in the study of complex projective dynamical systems.
